Urgency Annotations for Alternating Choices

We propose urgency programs, a new programming model with support for alternation, imperfect information, and recursion. The novelty are urgency annotations that decorate the (angelic and demonic) choice operators and control the order in which alternation is resolved. We study standard notions of contextual equivalence for urgency programs. Our first main result are fully abstract characterizations of these relations based on sound and complete axiomatizations. Our second main result settles their computability via a normal form construction. Notably, we show that the contextual preorder is (2h-1)-EXPTIME-complete for programs of maximal urgency h when the regular observable is given as an input resp. PTIME-complete when the regular observable is fixed. We designed urgency programs as a framework in which it is convenient to formulate and study verification and synthesis problems. We demonstrate this on a number of examples including the verification of concurrent and recursive programs and hyper model checking.

==> axioms_unused.tex <==

What is the coarsest congruence on program terms that preserves 
Eve’s winning region in every
urgency game that can be played over the grammar? 
%
The one that only imposes this requirement!
%
In the following definitions, we formalize this notion.


\begin{definition}
	Let $\objective\subseteq\analph^{*}$
	and $\aterm,\atermp\in\terms$.
	%
	The winning implication 
	$\aterm\specwinimpl{\objective}\atermp$ holds if 
	Eve winning $(\cfg, \objective)$ 
	from $\aterm$ implies Eve winning it from $\atermp$.
\end{definition}
\begin{definition}
	The specific winning precongruence
	$\speccongleq{\objective}\;\subseteq\terms\times\terms$
	is the largest precongruence within $\specwinimpl{\objective}$,
	that is $\aterm\speccongleq{\objective}\atermp$ 
	iff $\acontext{\aterm}\specwinimpl{\objective}\acontext{\atermp}$ for 
	all $\acontext{\contextvar}\in\contexts$.
\end{definition}

\begin{definition}
	The general winning precongruence
	$\congleq\;\subseteq\terms\times\terms$
	is the intersection of all specific winning precongruences 
	$\speccongleq{\objective\subseteq\analph^{*}}$.
\end{definition}

The intersection of all 
winning implications isn't enough to capture 
the congruence.
%
\color{green}
Reference the term at introduction
\color{black}

\subsection{Axiomatization}
We present two axiomatized precongruences.
%



Our main result is a full abstraction of the general winning 
implication $\winimpl$.
%
\begin{proposition}\label{Proposition:GeneralFA}
	$\axleq\;\scaleobj{0.92}{=}\;\congleq$.
\end{proposition}


Our result for the specific precongruence is
stated below.

\begin{proposition}\label{Proposition:SpecificFA}
	Let $\objective\subseteq\analph^{*}$.
	%
	We have 
	$\specaxleq{\objective}
	\scaleobj{0.92}{\subseteq}\speccongleq{\objective}$
	and if $\objective$ is right-seperating, then 
	$\specaxleq{\objective}=\speccongleq{\objective}$.
\end{proposition}


The axiomatization for the specialized contextual preorder needs the Myhill-
%
This precongruence uses the Myhill-Nerode (pre)congruence 
induced by the objective to further simplify the domain.
%

Our axiomatization of the specific congruence is 
a full abstraction only for certain objectives.
%
Namely, it is a full abstraction if the objective is 
right-seperating.
%
We call an objective $\objective\subseteq\analph^{*}$ 
right-seperating if the Myhill precongruence is 
equal to the right syntactic (in)equivalence.
%
This is formally stated in contraopposition form as follows:
%
\begin{definition}
	The objective $\objective\subseteq\analph^{*}$
	is called right-seperating 
	if for all 
	$\aword, \awordp\in(\analphbot)^{*}$ with
	$\aword\not\sgleq{\objective}\awordp$,
	there is a $\awordpp\in\analphbot^{*}$ 
	with $\aword\appl\awordpp\in\objective$ 
	and $\awordp\appl\awordpp\not\in\objective$.
\end{definition}

%
The proofs of the soundness directions 
$\axleq\scaleobj{0.92}{\subseteq}\congleq$
and 
$\specaxleq{\objective}\scaleobj{0.92}{\subseteq}
\speccongleq{\objective}$.
are given in \Cref{Section:Soundness}.
%


==> completeness_unused.tex <==
We thus have the following. 
These inclusions form the inclusion chain in 
\Cref{Corollary:CompletenessChain}.
%
This chain yields the desired completeness result 
$\axleq\;=\;\congleq$.

\begin{corollary}\label{Corollary:CompletenessChain}
	For domain shattering 
    $\objective\subseteq\analph^{*}$, we have
    $\congleq\;\subseteq\;\speccongleq{\objective}
	\;\subseteq\;\specaxleq{\objective}\;=\;\axleq\;
    \subseteq\;\congleq$.
\end{corollary}


    We prove that for all
    $\aterm,\atermp\in\gnfn{\maxurg}$, the statements
    $\aterm\discleq\atermp$, $\aterm\specaxleq{\objective}\atermp$,
    $\aterm\speccongleq{\objective}\atermp$, and 
    $\aterm\discleq\atermp$ imply one another.
    %
    Since we have already shown in \Cref{Section:Normalization} 
    that there are
    $\axeq$-equivalent terms in $\gnfn{\maxurg}$ for all terms,
    this is 
    sufficient for showing \Cref{Lemma:RightSeperating}.
    %
    The choice operators and $\specaxleq{\objective}$
    span a complete lattice on each urgency.
    %
    The implication from $\aterm\discleq\atermp$ to 
    $\aterm\specaxleq{\objective}\atermp$ follows from this 
    fact.
    %
    In \Cref{Section:Soundness}, we have already 
    shown the soundness of $\specaxleq{\objective}$,
    so $\aterm\specaxleq{\objective}\atermp$
    implies $\aterm\speccongleq{\objective}\atermp$.


==> complexity_mpdg.tex <==
\newcommand{\currcs}{\mathsf{k}}
\section{Lower Bound}
We prove the lower bound with a reduction from context-bounded multi-pushdown games, a concurrent programming model the complexity of which is well-understood~\cite{QadeerR05, MW20}. 
%
We see the fact that we can reflect this concurrency as another testament to the versatility of urgency annotations. 
% -------------------------------------------------------------------------
% -------------------------------------------------------------------------
% -------------------------------------------------------------------------
% -------------------------------------------------------------------------
\subsection{Multi-Pushdown Games}
We introduce multi-pushdown games in a variant that is trimmed to our needs. 
% 
A \emph{$\ctxtbound$-context-bounded 2-stack pushdown game~($\ctxtbound$-2PDG)} is a tuple $(\states, \evestates, \astate_0, \goalstates,  \Gamma, \transitions)$
consisting of a finite set of states~$\states$, 
a set of states $\evestates\subseteq\states$ owned by Eve, 
an initial state $\astate_0$, 
a set of goal states $\goalstates\subseteq\states$, 
a stack alphabet~$\Gamma$, and 
a set of transitions $\transitions\subseteq\states\times\stackops
\times\states$. 
%
Each transition is annotated by a stack operation from 
$\stackops=\Gamma\times\Gamma^{\leq 2}\cup\set{\nxt}$.
With operation~$(\asymbol, \aword)$, we pop $\asymbol$ from and 
push $\aword$ to the active stack.
With operation~$\nxt$, we change the active stack, also called a context switch. 
We assume there is a bottom of stack symbol $\stlsymbol\in\Gamma$ for both stacks
that is never removed. 
%We assume there are loops on all states and for all letters that prevent the game from deadlocking. 

The semantics of a $\ctxtbound$-2PDG is a game arena 
$(\configs, \to, \own)$ with a reachability objective $\configs_{\goalstates}$ for Eve.
%
The positions are configuration from 
$\configs=\states\times[0, \ctxtbound]\times\Gamma^{*}\times\Gamma^*$.
A configuration $(\astate, \currcs, s_1, s_0)$ stores the current state~$\astate$, 
the number of context switches~$\currcs$ that have occurred so far, and the contents of the two stacks. 
Stack $s_{0}$ is active after an even number of context switches, stack $s_{1}$ is active when $\currcs$ is odd.
The owner of the configuration is the owner of $\astate$. 
The moves between configurations are defined as expected. 
Note that there are no moves that would increase the number of context switches beyond $\ctxtbound$. 
We assume there are no deadlocks. %: there is always a transition enabled. 
%: Eve, in case $\astate\in\evestates$, and Adam otherwise. 
%
%The number of context switches is the number of A context switch 
%the changing of the current stack.
%
The objective is $\configs_{\goalstates}=\goalstates\times\set{\ctxtbound}\times\Gamma^{*}\times\Gamma^*$, 
meaning we reach a goal state and have exhausted the context switches.  
%
Plays, strategies, and winning are defined like for urgency games.
%
The task is to decide whether Eve has a strategy to win
from $(\astate_0, 0, \stlsymbol, \stlsymbol)$.
%
\begin{theorem}{\cite{MW20}}
    $\ctxtbound$-2PDG are $\kexptime{(\ctxtbound - 2)}$-complete.
\end{theorem}
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
\subsection{Reduction}
The reduction is in two steps, we first reduce 2PDG to the problem of making an observation:
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
\begin{proposition}\label{Proposition:LowerBound}
    Given a $(2\maxurg+1)$-2PDG $\pdg$, 
    we can compute in poly time 
    $\aterm$ over $\analph$ and  $(\nonterminals, \eqmap)$ of maximal urgency~$\maxurg$ and an objective DFA $\objective$ 
    so that Eve wins $\pdg$ if and only if $\winsof{\aterm}{\objective}$.
\end{proposition}

We now reduce the problem of making an observation to the specialized contextual equivalence. 
%
Indeed, $\winsof{\aterm}{\objective}$ is the same as to check $\whichcharof{\objective}{\contextvar} \speccongleq{\objective} \aterm$, where $\whichcharof{\objective}{\contextvar}$ is the characteristic term of the empty context formed for objective $\objective$. 
%
The problems is that the characteristic term may be exponential. 
%We know from \Cref{Lemma:CharTerm} that $\charof{\contextvar}=\bigAchoiceOf{1}\sizeof{\specgnfn{0}}$. 
%
%The problem is that $\sizeof{\specgnfn{0}}$ may be exponential.
%
We utilize the trick from \Cref{Section:CompactEncoding}. 
%
\begin{lemma}
Given $\aterm$ over $\Sigma$ and $(\nonterminals, \eqmap)$, and objective $\objective$. 
We can compute in poly time $\whichcharof{\arrof{\objective}}{\contextvar}$, $\arrof{\aterm}$, and $\arrof{\objective}$ so that $\winsof{\aterm}{\objective}$ if and only if $\charof{\contextvar} \speccongleq{\arrof{\objective}} \arrof{\aterm}$. 
\end{lemma}
The time bound is \Cref{Lemma:CharTerm} plus the size of the syntactic congruence for $\arrof{\objective}$. 
Correctness is \Cref{Lemma:DFASimulation}. 


In the remainder of the section, we sketch the proof of \Cref{Proposition:LowerBound}.
%We sketch a polynomial-time reduction from $(2\maxurg+1)$-2PDG to a term $\aterm$ with regular objective $\objective$.
%
We encode positions $(\astate, \currcs, \stsymboln{}\ldots\stlsymbol, 
\stsymbolpn{}\ldots\stlsymbol)$ of the given 2PDG as urgency terms of the form 
\begin{align*}
    \headerurg{\anurgpp}\appl
    \underbrace{\history\appl\wrpsymboln{}{\anurg}\ldots
    \wrplsymbol{\anurg}\appl\stacksep}_{s_1}
    \appl
    \underbrace{\historyp\appl\wrpsymbolpn{}{\anurgp}\ldots
    \wrplsymbol{\anurgp}\appl\stacksep}_{s_0}. 
\end{align*}
Stack symbols $\wrpsymboln{}{}\in\Gamma$ are represented by terms $\wrpsymboln{}{\anurg}$  
of urgency~$\anurg$.
%
Terminal symbol $\stacksep$ marks the end of a stack content encoding.
%
Also the terms $\history$ and $\historyp$ contain terminal symbols 
that represent the history of internal state changes in the 2PDG.\@
%
Finally, $\headerurg{\anurgpp}$ has urgency $\anurgpp$ and is used to guarantee 
continuity between the urgency levels.


The construction controls the urgencies $\anurgpp$, $\anurg$,
and $\anurgp$ tightly. 
%
After an odd number of context switches, the left stack is active and $\anurgpp+1=\anurg=\anurgp$. 
After an even number of context switches, the right stack is active and $\anurgpp+1=\anurg+1=\anurgp$.
This ensures the term encoding the top of the active stack is leading.
In either case, $\anurgpp+1 = \maxurg - \lfloor \currcs / 2 \rfloor$.

The top of the active stack allows the game to proceed as
\begin{align*}
    \ldots\history\appl
    \underbrace{(
        \Echoice{\astate\in\states}
        \Pchoice{\atrans\in\transitions_{\astate, \stsymboln{}}}
        \encoding{\atrans}^{\anurg}
    )}_{\text{Rewritten from }\wrpsymboln{}{\anurg}}
    \ldots\;\wrplsymbol{\anurg}\appl\stacksep\ldots
    \;\gamemove\;
    \ldots\history\appl\encoding{\atrans}^{\anurg}_{\stsymboln{}}
    \ldots\;\wrplsymbol{\anurg}\appl\stacksep\ldots
\end{align*}
%
Eve determines the current state  $\astate\in\states$ with a choice. 
%and fetching . 
%that fit the current state of the MPDG.
%
Then the player owning this state selects the next transition.  
%
We use $\transitions_{\astate, \stsymboln{}} \subseteq \transitions$ to denote the set of transitions
from state $\astate$ with top of stack symbol $\stsymboln{}$. 
The set is non-empty because the 2PDG does not deadlock.  
%
The term~$\encoding{\atrans}^{\anurg}$ of the chosen transition~$\atrans$
contains terminals which join history $\history$ to record the state change. 
%
Should Eve's choice of $\astate$ be inconsistent with the previous state, then this can be observed from $\history$. 
%
The history terminals %for in $\history$ (and $\historyp$ for the other stack) 
also remember the urgency~$\anurg$.
%}%
%, amongst other things, records Eve's decision about the current state in the history $\history$. 
%
%The corresponding letter not only reflects the chosen state, but also the current urgency. % in which the state has been generated.
%
The objective~$\objective$ is a product DFA that reads the terminals for each urgency separately and checks them for consistency with the 2PDA transitions. 
%
%The history is generated left to right 
%as long as the urgency does not change.
%
%So the DFA can recognize inconsistencies.
%
%Eve lose if the DFA detects a faulty move. 
%
For~$\winsof{\aterm}{\objective}$ to hold, Eve's choices must be consistent and lead to a goal configuration of the 2PDG.\@ 

If transition $\atrans$ pushes $\stsymbolpp$ or $\stsymbolpp_{0}\stsymbolpp_{1}$, the top of stack is rewritten accordingly ($\history'$ includes the new state change):
%
%If a pop-push transition is chosen, the top of stack symbol is directly rewritten into 
%the pushed string of symbols:
%
\begin{align*}
    \ldots\history\appl\makeleading{\wrpsymboln{}{\anurg}}\ldots 
    \wrplsymbol{\anurg}\appl\stacksep\ldots
    \;\;\gamemove\;\; 
    \ldots\history'\appl
        \makeleading{
        \wrpsymbolppn{}{\anurg}}
    \ldots 
    \wrplsymbol{\anurg}\appl\stacksep\ldots
\end{align*}
%
For a pop transition, the term to the right becomes leading and is the new top of stack.

To understand the rewriting process for $\nxt$-transitions, 
let us first explain the rewriting from $\wrpsymbol{\anurg}$ to 
${\atermpp = \Echoice{\astate\in\states}
\Pchoice{\atrans\in\transitions_{\astate, \stsymbol}}
\encoding{\atrans}^{\anurg}}$.
%
A stack symbol $\wrpsymbol{\anurg}$ is the term
${\encoding{\to\sty}^\anurg\appl\atermpp
\echoicen{\anurg}\encoding{\to\nxt}^\anurg\appl \wrpsymbol{\anurg-1}}$.
%
If Eve decides to proceed to $\atermpp$ as above, this is recorded in~$\history$ by a terminal $\encoding{\to\sty}^\anurg$.
%
Otherwise, she emits $\encoding{\to\nxt}^{\anurg}$ and effectively decrements the urgency by replacing $\wrpsymbol{\anurg}$ with $\wrpsymbol{\anurg-1}$. 


%Term $\atermpp$ initiates a choice for the next state and next transition as above.
%The terminals in $\encoding{\to\sty}$ record this .

If $\atrans$ is an $\nxt$-transition, then the leading term must swap the stack to emulate a context switch.
%
In that case, $\encoding{\atrans}^{\anurg}$ is the special terminal $\encoding{\nxt}^\anurg$
that informs the objective DFA about the context switch.
%
The DFA now expects to only see %no $\encoding{\to\sty}^\anurg$ to the right of $\nxt$, but only 
$\encoding{\to\nxt}^\anurg$ to the right.
%
This triggers a chain of moves in the encoding that decrements the urgency of every symbol on the now no longer active stack.
%
These moves use the alternative $\encoding{\to\nxt}^{\anurg}\appl \wrpsymbol{\anurg-1}$ in the aforementioned choice:
%
%
%
%The role of the emitted terminals~$\encoding{\to\nxt}$ is to let the DFA track the sequence of decrements.
%
%
%The following term illustrates the decrement process:
\begin{align*}
    &{
    \begin{tikzpicture}
        \draw[->] (0,0) -> node[above] {\footnotesize Progression of the leading term} (4,0);
    \end{tikzpicture}
    }\\[-0.5em]
    \ldots\history'\appl
    \encoding{\nxt}
    &\underbrace{\ldots
    \encoding{\to\nxt}\appl
    \wrpsymboln{i-1}{\anurg-1}}
    _{\text{Urgency }\anurg-1}\appl 
    \makeleading{\wrpsymboln{i}{\anurg}}
    \ldots\wrplsymbol{\anurg}\stacksep\ldots
\end{align*}
%
%
The DFA also forbids Eve to emit $\encoding{\to\nxt}^\anurg$ before $\encoding{\nxt}^\anurg$. 
%, which forces her to stay faithful with her choice.}
%
The terminal symbol $\stacksep$ resets the effect of $\encoding{\nxt}$ on the objective.

After the decrement process, if the left stack was active, the top of the right stack becomes the leading term. % since it is immediately to the right. 
%
If the right stack was active, all parts of the 
encoding have the same urgency and $\headerurg{\anurg-1}$ becomes leading.
%
Now, Eve has to guess the current state the 2PDA was in when leaving the context, and the objective verifies that the guess was correct. 
%
%This makes the history of the previous urgency visible to the DFA of the current urgency.
%
%After this, the top of the odd stack becomes leading.


Each urgency simulates two contexts, odd followed by
even.
%
Since we do not need to access the odd stack before the 
first context switch, we employ a construction 
that generates this stack when it is first accessed.
%
This allows us to simulate three contexts with the maximal urgency.
%
In total, the construction simulates $2\maxurg + 1$ contexts  with urgency $\maxurg$.


==> complexity_mpdg_unused.tex <==

\begin{comment}
%the set $\stackops$.
%
%In the usual definition, we have 
%$\stackops=\Gamma\times\Gamma^{\leq 2}\times\set{0, 1}$.
%
Here, the stack operation $(\asymbol, \aword, i)\in\stackops$ denotes 
popping $\asymbol$ from stack $i$ and pushing the string 
$\aword$ to the same stack.
%
Our definition is slightly different than, 
but equivalent to, the usual
definition.
% 
In our definition, each transition is annotated 
by an operation
$\stackops=\Gamma\times\Gamma^{\leq 2}\cup\set{\nxt}$.
%
The configurations of our game store information about 
the so called current stack.
%
All operations of the form 
$(\aletter, \aword)\in\Gamma\times\Gamma^{\leq 2}$ pop 
$\aletter$ and then push $\aword$ to the current stack.
%
The transitions annotated by
$\nxt$ make the next stack current.
%
Note that this is uniquely determined: In the case of two stacks,
there is always exactly one non-current stack.

%This represents the bottom of the stack.
%
Formally, 
if $(\stlsymbol,\aword)\in\stackops$, then the last symbol in 
$\aword$ is also $\stlsymbol$.
\end{comment}

%consists of the
%configurations where the first component, 
%the internal state, is in $\goalstates$.
%
The ownership assignment $\own:\configs\to\set{Eve, Adam}$ 
assigns each configuration to the owner of its internal state, 
so we have $\ownof{(\astate, i, s_{0}, s_{1})}=Eve$ if and only if 
$\astate\in\states_{E}$.
%
The successor relation makes the effects of the 
transitions formal.
%
It is the strictest 
relation that contains
$(\astate, n, s_{1}, s_{0})\to(\astatep, n+1, s_{1}, s_{0})$,
for all $(\astate, \nxt, \astatep)\in\transitions$,
and $(\astate, 2n-i, s_{1}, s_{0})\to(\astatep, 2n-i, s_{1}', s_{0}')$,
for all $(\astate, (\stsymbol, \aword), \astatep)\in\transitions$,
where $s_{i}=\stsymbol\appl\awordp$,
$s_{i}'=\aword\appl\awordp$, and 
$s_{1-n}'=s_{1-n}$ for some $\awordp\in\Gamma^{*}$.
%
Remark that since we only have two stacks, the amount of
context switches uniquely determines the current stack, 
given that the initially current stack is fixed.
%
Here, the stack $s_{0}$ is current after an even amount of context switches.
%
Conversely,  the stack $s_{1}$ is current after an odd amount of 
context switches.
%
We call these stacks even and odd stacks respectively.
%
Strategies, winners and plays are defined analogously
to those from urgency games.
%
The question we are
interested in is 
whether Eve has a winning strategy 
from the position $(\astate, 0, \stlsymbol, \stlsymbol)$, 
meaning the play starts in the initial state 
with both stacks empty. 
%
Per se, this problem is undecidable.


%To keep the construction simple, we say that Eve only wins if she reaches 
%a final state after exhausting all contexts.
%
%Formally, we restrict 
%Eve's reachability objective to $
\goalstates\times\set{\ctxtbound}\times\Gamma^{*}\times\Gamma^{*}$.
%
We further restrict ourselves to MPDG which cannot deadlock:
%
For any configuration $\aconfig\in\configs$ 
with $<\mathrm{b}$
context switches, there is a 
$\aconfigp\in\configs$ with $\aconfig\to\aconfigp$.



==> introduction_unused.tex <==


The latter term in the above equationsterm resulting from the two equations indeed is in normal form.
%
We then employ the notion of characteristic contexts
We then reduce completeness for the contextual equivalence to completeness of the specialized variant. 
This notion of completeness is then proven
 sound and complete axiomatization of the two relations.

 and an axiomatization
 we relate two programs for every possible 

 follow the established lines
a choice of granularity at which to observe the behavior of the program.
We  


As common in contextual equivalence, there is a choice in the granularity of the observation that the environment can make.  
A

study urgency from a semantic perspective what is the notion of contexual equivalence  
Our contribution is a semantic study of the contextual equivalence for 


allows us to give an easy embed without effort, 
With higher urgencies, the same idea allows us to e idea car

For example, the only difference between simulation and language inclusion problems betwee




We developed urgency annotations to make explicit an observation that we believe is folklore: 
several problems in verification have a com: they rely on an alternating programming model and the only difference are the rules according to verification problems have alternation as a common basis, and the only difference between them are the rules according to which the choices are resolved.
Urgency annotations make explicit this these problems in a single, unified programming model. 
Consider simulation and language inclusion problems between finite-state systems $A$ and $B$.
In both problems, a demonic choice for the next transition in $A$ has to be matched by an angelic choice for the next transition in $B$. 
The only difference is that in simulation problems the choices have the same urgency. 
In language inclusion problems, the demonic choices of $A$ have a higher urgency than the angelic choices of $B$. 
The word has to be generated entirely before $B$ has to decide for an accepting run.
With higher urgencies, it is poss
The argument carries over to 

 , because the word has to be gen, howeveover a Simulation problems require a single urgency, the demonic choice for a transition in the left  make visible 
, for example, 
The difference between simulation and language-inclusion problems, for example, 



  like perfect and imperfect information games or simulation and language-inclusion problems between all rely on hte 


a variety of computational model

the difference between s
there are well-known programming models that 
programming models
a variety of programming models is 

from the folklore feeling models of computation 

have the same underlying basis, namely a programming model with alternation, and the only difference are the rules according to which the choices are revealed. 
The first example captures perfect-information games or simulation problems. 
With a higher urgency as in the second example, we can 

  and w are motivated by the fact that  stems from the observation that well-known models of computation can be traced back to an alternating programming model honly differ in the  various models of computation 
can be formulated as alteranting choices that 
only di can be formulated in a uniform way: the only difference is in the actual urgency annotation.
The above example captures the difference between simulation problems between finite-state systems and language inclusion. 
From here to hyper. 



Consider the program $(\aletter_1 \achoicen{1}\aletterp_1).(\aletterpp_1\echoicen{i}\aletterppp_1).(\aletter_2\achoicen{1}\aletterp_2).(\aletterpp_2\echoicen{i}\aletterppp_2)$ and assume $i=1$.
%
Then the players take turns to produce a word
\begin{align*}
(\aletter_1 \achoicen{1}\aletterp_1).(\aletterpp_1\echoicen{i}\aletterppp_1).(\aletter_2\achoicen{1}\aletterp_2).(\aletterpp_2\echoicen{i}\aletterppp_2) 
\end{align*}
The need for urgency annotations stems from the observation that well-known models of computation can be formulated in a uniform way: the only difference is in the actual urgency annotation.
The above example captures the difference between simulation problems between finite-state systems and language inclusion. 
From here to hyper. 

Our contribution 

We start from the observation that several problems in verification have
the same computational phenomenon: 
they equip alternating choices with a degree of visibility.
Take the question of whether a finite state system simulates another one.
The problem can be modeled by a demonic choice for a transition in $A$ followed by a a product system in which the 
Take
alternating (angelic and demonic) choices that are executed in a round based fashion 
made visible with delay.
Consider perfect




Our study starts from the observation that apparently different models of computation 
rely on the same basic mechanism that is implemented in a diffenre: alternating (angelic and demonic) choices, an

only differ in the way they use a basic mech

rely on the same basic mechanism: they endow choice operators with a notion of visibility. 
We propose to make this mechanism explicit as a new 
























What is the need?
The interplay between imperfect information and recursion is not well-understood. 
Imperfect information already means two parties. 

Study of contextual equivalence received considerable attention. 
Focus has been on programming models with higher-order features and recently concurrency. 
Alternation not been tackled.
Hiding not been tacke

Imperfect information and recursion are not well-understood. 

==> normalization_unused.tex <==

Note that normal forms are built by 
subset construction.
%
%
For the rest of this section, fix an objective 
$\objective\subseteq\analph^{*}$.


This is done by normalizing the terms 
recursively.
%
For all such $\bigPchoiceOf{\anurg}\atermset\in\terms$ and 
$\aterm\appl\atermp\in\terms$ where the 
function is not yet defined, we let 
$\normof{\aterm\appl\atermp}=0
\normof{\normof{\aterm}\appl\normof{\atermpp}}$ 
and 
%$\normof{\bigPchoiceOf{\anurg}\atermset}=\normopof{
 %   \bigPchoiceOf{\anurg}
  %  \set{\normof{\aterm'}\mid \aterm'\in\atermset}}$.
%
We construct the function by first handling base cases, namely operations on normal form terms.
%
We then generalize the process to all terms that do not contain non-terminals.
%
This allows us to perform (transfinite) least fixed point calculations to normalize 
all non-terminals.
%
Augmenting the construction by a base case for non-terminals,
we obtain complete normalization schemes.



==> optimal_decidability_unused.tex <==
We turn to the algorithm for 
\decwhichover{\speccongleq{*}}{\maxurg}. The goal is:
%

%
Since our specialized axiom system is not complete for 
arbitrary regular objectives, the algorithm exhaustively checks  
the winner for all contexts.
%
Deciding $\winsof{\aterm}{\objective}$ for $\aterm\in\specgnfn{\maxurg}$ is done in bottom-up fashion in time polynomial in $\sizeof{\aterm}$.



We turn to the algorithm for \Cref{Proposition:DecideUpperBoundEff}.
The task of checking the winner under all contexts
is simplified
by the use of \Cref{Lemma:ContextLemma}, which states 
that only immediate contexts need to be checked.
%
\Cref{Proposition:EffNormalForm} further alleviates the task: Each context is transformed into one of shape
$\contextvar$, 
$\atermppp\appl\contextvar$, 
$\contextvar\appl\atermpppp$, or 
$\atermppp\appl\contextvar\appl\atermpppp$, 
where $\atermppp\in\specgnfn{\maxurg-1}$ and $\atermpppp\in\specgnfn{\maxurg}$.



\Cref{Theorem:UpperLowerInput} promises a $\kexptime{(2\maxurg-1)}$ upper bound.
%
But doing an exhaustive search over all stated contexts takes too long.
%
For an arbitrary objective $\objective$, 
$\sizeof{\specgnfn{0}}$ is already $\expof{1}{\sizeof{\objective}}$
and thus
$\expof{2\maxurg-1}{\bigoof{\sizeof{\specgnfn{0}}|}}
\sim\expof{2\maxurg}{\bigoof{\sizeof{\objective}}}$.
%
Creating a normal form is already too expensive.
%
Further, $\sizeof{\specgnfn{\maxurg}}=\expof{2\maxurg}{\sizeof{\specgnfn{0}}}$.
%
So even if $\sizeof{\specgnfn{0}}$ were polynomial in $\sizeof{\objective}$, 
an algorithm that iterates over all $\atermpppp\in\specgnfn{\maxurg}$ 
would not be in $\kexptime{(2\maxurg-1)}$.
%
To satisfy \Cref{Proposition:DecideUpperBoundEff}, we need a more sophisticated approach.




First, we handle the uncomfortable size of $\specgnfn{0}$.
%
It is commonly known, that a class of $\lreq{\objective}$ is representable by a function of states to states $\aclass : \states \to \states$ of the minimal DFA~\cite{todo}.
%
The key insight is to let Eve simulate the effect of the terminals $\aclass \in \analphbot^*/\lreq{\objective}$ on the DFA by letting her choose one pair of states.


\begin{gather*}
    \arrof{\aletter}=\bigEchoiceOf{1}{}{\setcond{(\astate, \astatep)}
        {\transitions(\astate,\aletter) = \astatep}} \\

\end{gather*}


is a term over $\arralph$ and $(\nonterminals, \arreqmap)$ with
%
With a representative system for the syntactic congruence, we can assume the alphabet is still $\analphbot$. 


The new objective is the set of accepting DFA runs 
${\arrobjective=
\setcond{(\astatep_0,\astate_{1})(\astate_{1}, \astate_{2})\ldots
(\astate_{n}, \astate_{n+1})}{\astate_{n+1}\in\goalstates}}$.
%
In order to keep such a construction correct, her choice needs to know the DFA-run up to the current position in the term. 
%
An urgency of 1 for the choice will accomplish this task:
%
Whenever a terminal $\aclass \in \analphbot^*/\lreq{\objective}$ is to be generated, 
the game instead generates the term 
$\bigEchoiceOf{1}{}{\setcond{(\astate, \astatep)}{\transitions(\astate,\aletter) = \astatep}}$.
%
Because of its urgency, this choice is resolved 
only when there is a string of~$\arralph$ elements to its left.
%
The string of terminals represents a run on the DFA.
%
If Eve ever chooses $(\astate, \astatep)\in\arralph$ where 
$\astate$ is not the latest state in this run, 
she can never reach $\arrobjective$.



We identify a subset of plausible terms $\plgnfn{\anurg} \subset \specgnfnof{\anurg}{\arrobjective}$ and $\plagnfn{\anurg} \subset \specagnfnof{\anurg}{\arrobjective}$ for each $\anurg$.
%
As a matter of fact, we construct them so that $\plgnfn{1}$ contains precisely terms $\atermpp$ in normal form which have equivalent $\arrof{\atermpp'}$ with $\atermpp' \in \specgnfn{1}$:
%
\begin{align*}
    \plgnfn{0} &= \specgnfnof{0}{\arrobjective} & \plgnfn{1} &= \normof{\arrof{\specgnfn{1}}} \subset \specgnfnof{1}{\arrobjective}\,.
\end{align*}
%
We construct the higher urgency $\anurg > 1$ normal forms the same as before: 
${\plagnfn{\anurg+1}=\setcond
        {\bigAchoiceOf{\anurg}{}{\atermset}}
        {\emptyset\neq\atermset\subseteq\plgnfn{\anurg}}}
$
and  
${\plgnfn{\anurg}=\setcond{\bigEchoiceOf{\anurg}\atermset}
        {\emptyset\neq\atermset\subseteq\plagnfn{\anurg}}}
$.
This lets us identify the contexts to iterate over. 
\[
    \arrcontexts=
    \setcond{\contextvar, 
        \atermppp\appl\contextvar, 
        \contextvar\appl\atermpppp,
        \atermppp\appl\contextvar\appl\atermpppp} 
    {\atermppp \in \plgnfn{\maxurg-1}, \atermpppp \in \plgnfn{\maxurg}}\,.
\]



The proposition resolves the first issue:
%
We ensured ${\sizeof{\plgnfn{0}} = \sizeof{\specgnfnof{0}{\arrobjective}}\leq \sizeof{\objective}^{2}}$,
so we have avoided the first exponentiation.
%
But we still need to iterate over ${\sizeof{\arrcontexts} = \sizeof{\plgnfn{\maxurg-1}}\cdot\sizeof{\plgnfn{\maxurg}}}$ contexts 
and $\sizeof{\plgnfn{\maxurg}}$ is $2\maxurg$-exponential in $\sizeof{\objective}$.
%
We need a faster iteration of the contexts. 

We solve the second issue by \emph{characterizing} contexts. 
%
What does a context $\acontext{\contextvar}$ do for $\speccongleq{\objective}$?
%
It proves $\aterm \not \speccongleq{\objective} \atermp$ for terms, where $\winsof{\acontext{\aterm}}{\objective}$ holds but $\winsof{\acontext{\atermp}}{\objective}$ does not hold.
%
Indeed, we characterize $\acontext{\contextvar}$ by the set of terms $\aterm$ where $\winsof{\acontext{\aterm}}{\objective}$.
%
Even better, we find a term $\charof{\acontext{\contextvar}} \in \terms$ to do the job.

We give Adam the choice on how he wants to lose the game by setting $\Achoice \setcond{\aterm}{\winsof{\acontext{\aterm}}{\objective}}$. 
%
But we need to understand the urgencies for the choice and which terms $\aterm$ the set needs to consider.
%
We find that there is a finitary characteristic term, and it is relatively small, too.
%



    %$\expof{2\maxurg-1}{\bigoof{\sizeof{\states}^2}}$. 
    %first a normalization of 
    %$\winsof{\acontext{\aterm}}{\arrof{\objective}}$ takes time 
    %$\sizeof{\acontext{\aterm}} \cdot \expof{2\maxurg-1}{\bigoof{\sizeof{\states}^2}}$, 
    %and $\sizeof{\acontext{\aterm}} \leq 3 \cdot \sizeof{\specgnfnof{\maxurg}{\arrobjective}}= \expof{2\maxurg-1}{\bigoof{\sizeof{\states}^2}}$.

 definition is correct and 
That this is the right definition is
The terms to lose with are taken from $\specgnfnof{\maxurg-1}{\arrof{\objective}}$, 
and thus the characteristic term is from $\specagnfnof{\maxurg}{\arrof{\objective}}$. 
This set is exponentially smaller than $\arrcontexts$.  

    \\
    \charof{\contextvar\appl\bigEchoiceOf{\maxurg}{}{\atermsetpppp}}
    & \disceqof{\arrobjective}
    \normof{\bigAchoiceOf{\maxurg}{}{
        \setcond{\charof{\contextvar\appl\atermpppp}}
            {\atermpppp\in \atermsetpppp}}}\,,
    \label{Equation:CharTermRecursive2}



consider a term $\aterm = \bigEchoiceOf{\maxurg}_{i\in I}{\bigAchoiceOf{\maxurg}{}{\atermset_i}}$ with $\winsof{\acontext{\aterm}}{\arrof{\objective}}$.
%
Since Eve wins, there is $i\in I$ so that for all $\atermp \in \atermset_i$, there is $\atermpppp \in \atermsetpppp$ with $\winsof{\atermppp\appl\atermp\appl\atermpppp}{\arrof{\objective}}$, which means\ $\charof{\atermppp\appl\contextvar\appl\atermpppp} \speccongleq{\arrof{\objective}} \atermp$. 
 and vice versa.\svdwf{The vice versa part is not easy to see. Make a lemma out of it and prove?}


This yields the following: 


We add them 
We only add the new terms if 
Then we conjoin the cha
What saves us is that we know there are at most $\expof{2\maxurg-1}{\bigoof{\sizeof{\objective}^2}}$ characteristic terms.
%
We can thus construct the characteristic terms for the subsets in a fixed point iteration

The result of \Cref{Equation:CharTermRecursive,Equation:CharTermRecursive2} is that the iteration of $\arrcontexts$ can be done fast enough.
%
We define for any sets of terms $\atermsetppp\subseteq\specgnfnof{\maxurg-1}{\arrobjective}$ 
    and $\atermsetpppp\subseteq\specagnfnof{\maxurg}{\arrobjective}$
    the set 
\[
    \allchartermsof{\atermsetppp}{\atermsetpppp}=
    \bigcup_{{\atermppp\in\atermset, \atermsetpppp\subseteq\atermsetp}}
    \set{
        \charof{\atermppp\appl\contextvar}, 
    \charof{\contextvar\appl\bigEchoiceOf{\maxurg}{}{\atermsetpppp}},
    \charof{\atermppp\appl\contextvar\appl\bigEchoiceOf{\maxurg}{}{\atermsetpppp}
    }}
\]

\begin{comment}
    With this at hand, 
we finally prove \Cref{Proposition:DecideUpperBoundEff}.

\begin{proof}[Proof of \Cref{Proposition:DecideUpperBoundEff}]
    First, we construct $\arrof{\aterm}$,
    $\arrof{\atermp}$ and $\arreqmap$.
    %
    We have that $\sizeof{\arrof{\aterm}}\leq \sizeof{\objective}\sizeof{\aterm}$,
    $\sizeof{\arrof{\atermp}}\leq \sizeof{\objective}\sizeof{\atermp}$, and 
    $\sizeof{\arreqmap}\leq \sizeof{\objective}\sizeof{\eqmap}$ by the nature of 
    the construction.
    %
    We apply the normalization algorithm from 
    \Cref{Proposition:EffDenSemUpperBound} 
    to get $\aterm'\specaxeq{\arrobjective}\arrof{\aterm}$ and 
    $\atermp'\specaxeq{\arrobjective}\arrof{\atermp}$.
    in 
    $(\sizeof{\objective}\sizeof{\aterm}+\sizeof{\objective}\sizeof{\eqmap}|\nonterminal|
    +\sizeof{\objective}\sizeof{\atermp})
    \cdot\expof{2\maxurg-1}{\bigoof{\sizeof{\objective}^{2}}}$
    time since $\sizeof{\specgnfn{0}}\in\bigoof{\sizeof{\objective}^{2}}$.
    %
    Now acquire
    $\chi(\plausiblectx)$ in 
    $\expof{2\maxurg-1}{\bigoof{\sizeof{\objective}^{2}}}$ time
    using \Cref{Lemma:CharTermsAtScale}.
    %
    We have that $\winsof{\acontext{\aterm}}{\arrobjective}$ 
    implies $\winsof{\acontext{\atermp}}{\arrobjective}$ for all 
    $\acontext{\contextvar}\in\plausiblectx$
    if 
    and only if for all $\atermppppp\in \chi(\plausiblectx)$, 
    $\atermppppp\discleq\aterm'$ implies
    $\atermppppp\discleq\atermp'$.
    %
    Per \Cref{Proposition:PlausibleNormalContexts}
    this is equivalent to $\aterm\speccongleq{\objective}\atermp$.
    %
    Checking whether $\bigEchoiceOf{\maxurg}\atermppppp\discleq\atermpp$ for 
    $\atermpp\in\specgnfnof{\maxurg}{\arrobjective}$ and 
    $\atermppppp\in\specagnfnof{\maxurg}{\arrobjective}$
    can be done in
    $\expof{2\maxurg-1}{\bigoof{\sizeof{\objective}^{2}}}$ time.
    %
    Since $|X|\subseteq|\specagnfn{\maxurg}|$,
    we have that $|X|\leq\expof{2\maxurg-1}{\sizeof{\objective}^{2}}$.
    %
    So iterating over all $\atermppppp\in X$ and performing the 
    check takes $(\expof{2\maxurg-1}{\bigoof{\sizeof{\objective}^{2}}})^2
    =\expof{2\maxurg-1}{\bigoof{\sizeof{\objective}^{2}}}$
    time.
    %
    This completes the proof.
\end{proof}
\end{comment}


==> preliminaries_before_rewrite.tex <==
\section{Urgency Games}
We propose urgency games as a programming model with support
for alternation and recursion.
What is new in this model is a programming construct called urgency
whose purpose is to control the order in which choices have to be revealed.
We propose natural notions of contextual equivalence the study of which
is the contribution of this work.

\subsection{Syntax}
Let $\maxurg>0$ be a natural number and let $\analph$ be a (finite) alphabet.
  
An $\maxurg$-\emph{urgency grammar} over $\analph$ is a pair
$\cfg = (\nonterminals, \eqmap)$ consisting of a not necefinite set of non-terminal symbols $\nonterminals$ and a function $\eqmap$ mapping
each non-terminal to a $\maxurg$-urgency term built from 
the set $(\analph\cup\set{\bot})\cup\nonterminals$.
%
The symbol $\bot$ is a fresh terminal symbol not contained in 
$\analph$.
%
We write $\analphbot=\analph\discup\set{\bot}$.
%
A $\maxurg$-urgency 
term built from the set $\analphbot\cup\nonterminals$
is a symbol $s\in\analphbot\cup\nonterminals$,
a concatenation of two terms, or
a $\anurg$-urgency choice 
of a set of terms $\atermset\neq\emptyset$
that belongs to a player, where $0<\anurg\leq\maxurg$.
%
We write $\aterm\achoicen{\anurg}\atermp$ and 
$\aterm\echoicen{\anurg}\atermp$ to denote
the binary choices $\bigEchoiceOf{\anurg}\set{\aterm, \atermp}$ 
and $\bigAchoiceOf{\anurg}\set{\aterm, \atermp}$.
%
\begin{align*}
    \aterm ::= s \mid \aterm\appl\aterm
    \mid  \bigEchoiceOf{\anurg}\atermset \mid \bigAchoiceOf{\anurg}\atermset
\end{align*}
%
A term can contain a choice of any set of terms.
%
Therefore the collection of all $\maxurg$-urgency terms
does not formally form a set.
%
Working with sets is essential 
for the sound application of game theoretical 
concepts.
%
For this reason, we restrict
the structural depth of the terms we work with 
by some fixed ordinal.
%
Structural depth of a term is defined in the usual way.
%
We let $\dpthof{\nonterminal}=\dpthof{\aletter}=0$ 
for all $\aletter\in\analphbot$ and $\nonterminal\in\nonterminals$.
%
The depth of a choice term or a concatenation term is 
the smallest ordinal, greater than the depths of all the operands.
%
We also assign a depth to the entire grammar 
$\cfg=(\nonterminals, \eqmap)$.
%
The depth of a grammar
$\cfg=(\nonterminals, \eqmap)$ 
is defined to be the smallest non-zero 
limit ordinal larger than 
$\dpthof{\eqmapof{\nonterminal}}$ for all $\nonterminal\in\nonterminals$.
%
We denote this by $\dpthof{\cfg}$.
%
The set of terms constrained by $\cfg$ is 
$\terms_{\cfg}=\set{\aterm\in\terms\mid 
\dpthof{\aterm}<\dpthof{\cfg}}$.
%
For the rest of this paper,
we only focus on terms $\terms_{\cfg}$ when dealing with 
the grammar $\cfg$.

A context $\acontext{\contextvar}$ from an                                                                                                                                                                                                                                          $\maxurg$-urgency grammar 
$\cfg=(\nonterminals, \eqmap)$ is a term of the 
$\maxurg$-urgency grammar 
$\cfg'=(\nonterminals\discup\set{\contextvar}, \eqmap)$
with at most one occurrence of the fresh non-terminal 
$\contextvar$.
%
The set of all contexts is denoted $\contexts_{\cfg}$.
%
The expression $\acontext{\aterm}$ refers to the term 
acquired by replacing the non-terminal $\contextvar$ 
by the term $\aterm$.
%
This replacement operation is well defined within $\terms_{\cfg}$.

\begin{lemma}\label{Lemma:SensibleOrdinal}
    Let $\cfg=(\nonterminals, \eqmap)$ be an $\maxurg$-urgency grammar.
    %
    Then, for all $\aterm\in\terms_{\cfg}$ and 
    all 
    $\acontext{\contextvar}\in\contexts_{\cfg}$,
    we have
    $\acontext{\aterm}\in\terms_{\cfg}$.

\end{lemma}

We employ the symbol $\pchoicen{\anurg}$ 
to denote one of the choices $\echoicen{\anurg}$ and
$\achoicen{\anurg}$.
%
A term $\atermp$ is called a subterm of $\aterm$ 
if there is a context 
$\acontext{\contextvar}$ 
with $\aterm=\acontext{\atermp}$.
% 
A subterm is called outermost 
if it isn't enclosed by a choice.
%
For example, $\aterm$ is outermost in $\aterm\appl\atermp$ 
but not in $(\aterm\echoicen{\anurg}\atermp)\appl\atermpp$.
%
An outermost action is an outermost subterm that 
doesn't have choice or
concatenation as its outermost operator.
%
Remark that all terms are the concatenation of their 
outermost actions.

An $\maxurg$-urgency grammar $\cfg = (\nonterminals, \eqmap)$
induces a rewriting relation 
$\to\subseteq\terms_{\cfg}\times\terms_{\cfg}$.
%
To define this relation, we first need to lift the notion of urgency 
from the choices to terms.
%
The \emph{urgency} of a term is defined to be the highest urgency 
of its outermost actions.
%
We formalize this by the following function 
$\urgency: \terms_{\cfg}\to\nat$:
%
\begin{align*}
    &\urgencyof{\aletter}=0\qquad
    \urgencyof{\nonterminal}=\maxurg\qquad
    % 
    \urgencyof{\bigPchoiceOf{\anurg}\atermset}=\anurg\\
    &\urgencyof{\aterm\appl\atermp}=max\set{\urgencyof{\aterm}, \urgencyof{\atermp}}
\end{align*}
%
The rewriting relation always rewrites the \emph{leading 
subterm}.
%
The leading subterm $\leadingof{\aterm}$ of $\aterm$
is defined as the outermost 
action with the highest urgency.
%
If there are multiple such subterms, then the leftmost of these is 
leading.
%
We denote a subterm that contains the leading term 
by an underline (e.g. $\aterm\appl\makeleading{\atermp}$).
%
Note that for $\makeleading{\aterm}\appl\atermp$ and 
$\aterm\appl\makeleading{\atermp}$, we have 
$\urgencyof{\aterm}\geq\urgencyof{\atermp}$
and $\urgencyof{\atermp}>\urgencyof{\aterm}$ respectively.
%
We denote the unique context enclosing the leading term
$\leadingof{\aterm}$
in $\aterm$ by $\enclosingctx{\aterm}{\contextvar}\in\contexts_{\cfg}$.
%
The rewriting operation replaces one term enclosed in a context.
%
So per \Cref{Lemma:SensibleOrdinal},
this relation is also well defined in $\terms_{\cfg}$.
%
To clear up the notation in the rest of the paper, we 
define $\successorsof{\aterm}=\set{\aterm' \mid \aterm\to\aterm'}$.
%
The rewriting relation $\to$ is formally defined as the strictest 
relation that satisfies the rules below.
%
\begin{align*}
    \axdef{}{}{\bigPchoiceOf{\anurg}\atermset\to\aterm}
    \qquad
    \axdef{}{}{\nonterminal\to\eqmapof{\nonterminal}}
    \qquad
    \axdef{}{\leadingof{\aterm}\to\atermp}
    {\aterm
    \to\enclosingctx{\aterm}{\atermp}}
\end{align*}
%
\subsection{Game Semantics}
The semantics of an urgency grammar $\cfg$ is the (typically
infinite) game arena $[[\cfg]]=(\terms_{\cfg}, \to, \own)$.
%
The ownership assignment returns the owner of the leading subterm,
so $\ownof{\aterm}=\ownof{\leadingof{\aterm}}$.
%
The choices are owned by the respective players, 
while the non-terminals are owned by Eve.
%
Formally, 
$\ownof{\bigEchoiceOf{\anurg}\atermset}=\ownof{\nonterminal}=
\ownof{\aletter}=Eve$
(for all $\nonterminal\in\nonterminals$, 
$\aletter\in\analphbot$)
and 
$\ownof{\bigAchoiceOf{\anurg}\atermset}=Adam$.


Note that we give the ownership of non-terminals and terminals
to Eve.
%
This does not matter as the positions have at most one successor. 
%
It is worth noting
that the arena has perfect information, 
all choices are eventually revealed.
%
An $\maxurg$-urgency game $(\cfg, \objective)$
endows the $\maxurg$-urgency grammar $\cfg$ over the alphabet $\analph$
with a so-called
reachability objective $\objective\subseteq\analph^{*}$.
%
We use this set as the
reachability objective in the arena $[[G]]$.
%
The game-theoretic notions are as expected.
%
A play is a
maximal (finite or infinite) sequence of positions 
$\aplay=\aterm_{0}, \aterm_{1}, ...$
that respects the edges of the game,
$\aterm_{i}\to\aterm_{i+1}$ for all $i$. 
%
The play is won by Eve if it reaches a string of terminals 
$\aterm$ with $\aterm\in\objective$. 
%
Note that strings of terminals do not admit further rewriting. 
%
A (positional) strategy for Eve is
a function $\strat: \terms_{\cfg}\to\terms_{\cfg}$
so that $\aterm\to\strat(\aterm)$
for all terms $\aterm$ owned by Eve that admit further rewriting.
%
As we have
a reachability game, we can use positional strategies 
without loss of generality~\cite{Martin75}. 
%
A play $\aplay$ is conform to $\strat$ if 
for all $i$ with $\ownof{\aterm_{i}}=Eve$.
we have $\strat(\aterm_{i})=\aterm_{i+1}$.
%
Eve wins $(\cfg, \objective)$ from $\aterm$, if she
has a strategy $\strat$ that allows her to win all plays
starting in $\aterm$ that are conform to $\strat$. 
%
The set of all winning positions is Eve’s winning region.

We can also have a bound on the number of turns 
in which Eve can force a win.
%
Because our game graph has infinite outgoing degree,
this bound is expressed in the form of an ordinal, 
formalized by the following lemma.
%
Note that for $\aterm\in W$, if 
$\ownof{\aterm}=Adam$ then $\successorsof{\aterm}\subseteq W$.
\begin{lemma}\label{Lemma:WinBound}
    Let $\cfg=(\nonterminals, \eqmap)$ 
    and let $(\cfg, \objective)$ be an urgency game
    where $W\subseteq \terms_{\cfg}$ is Eve's winning 
    region.
    %
    Let $\anordinal$ be the smallest (limit) ordinal 
    with cardinality larger than $\terms_{\cfg}$.
    %
    Then, there is a mapping $f:W\to \anordinal$ 
    such that 
    $f(\aterm)=\inf\set{f(\atermp)+1 \mid \atermp\in W\cap\successorsof{\aterm}}$
    if $\ownof{\aterm}=Eve$ 
    and $f(\aterm)=\sup\set{f(\atermp) + 1\mid
     \atermp\in W\cap\successorsof{\aterm}}$
    if $\ownof{\aterm}=Adam$.
\end{lemma}

For the remainder of the paper, 
we fix a $\maxurg$-urgency grammar to 
$\cfg=(\nonterminals, \eqmap)$ over an 
alphabet $\analph$.
%
We also drop the $\cfg$ subscripts in 
$\terms_{\cfg}$ and $\contexts_{\cfg}$.

==> preliminaries_unused.tex <==
We use $\terms$ to refer to the set of all terms of urgency $\maxurg$ over $\analph$ and $\nonterminals$. 
%
To implement the recursion, we assume the set of non-terminals comes with a function $\eqmap:\nonterminals\to \terms$ that assings to each non-terminal $\nonterminal$ a so-called defining term $\eqmapof{\nonterminal}$. 
%
Throughout the development, we will fix $\maxurg$, $\analph$, and $\nonterminals$. 


An \emph{$\maxurg$-urgency grammar} over $\analph$ is a pair
$\cfg = (\nonterminals, \eqmap)$ consisting of a (not necessarily finite) set of non-terminal symbols $\nonterminals$ with $\nonterminals\cap \analph=\emptyset$ and a function~$\eqmap$ mapping
each non-terminal to an $\maxurg$-urgency term, also called the defining term. 
%

%
, 
%
We motivate the use of infinitary syntax in a moment. 
%

==> related_unused.tex <==

 where hyper model  makes a difference for computability when recursion comes into play:
problems like making an observation or contextual equivalence 
when formulating hyper model checking as urgency programs, we show that hyper pr problems remain decidable  
While this is no limitation in the finite-state case, it leads to decidability results for urgency programs where hyper model checking is undecidable. 

Indeed, a recent undecidability result for hyper model checking visibly pushdown systems shows that the synchronization among words required for 
 (right-linear) does not make a difference in the finite %while the words in 
%By executing choices out-of-program-order, urgency programs can indeed determine more than one run of the same system. 
%The additional runs can be chosen arbitrarily, as long as the system is finite state. 
%In the recursive case, however, our model is less liberal in the selection of runs, because 
%the urgent choices are harmonized with the control flow. 
This 
This is the advantage of urgency programs over hyper model checking. 
The model is constrained enough to obtain decidability results in the presence of recusion, 
yet practical that is practically still useful, but admits more new decidability resuts in the presence of recursion.  
%that the urgent choices are harmonized with the control flow.  
%we obtain decidability results in the presence of recursion. 
% challenging as contextual equivalence over  
%We obtain decidability results for problems as  in the presence of recursion. % new decidability results for checking hyper properties over recursive programs. % where hyper model checking is undecidable. 
Hyper model checking, in turn,  was shown to be undecidable even for visibly pushdown systems, intuitively, because the existing models fail to sufficiently synchronization the selection of words. 
We argue in the appendix that our assumption of sharing the control flow is also worthwhile in practice. 

Related work on contextual equivalence.

Related work on deciding contextual equivalence. 

Related work on full abstraction results/denotational semantics. 

Related work on axiomatization.

Related work on imperfect information. 


The idea of urgencies goes back to the recent work on hyper properties 
for expressing security requirements.
A hyper property $\aprop$ for a language $\alang$ over an alphabet $\analph$ takes the form of an alternation
\begin{align*}
\forall \aword_1\in \alang.\ \exists \aword_2\in\alang\ \ldots\ \mathit{Q} \aword_n\in \alang_n.\ \aword_1\oplus\ldots \oplus \aword_n\in \aprop\ .
\end{align*}
Here, $\oplus$ is the convolution and $\aprop$ is a language over~$\analph^n$.
The standard way of model checking hyper properties is by a repeated composition of the system generating $\alang$ with itself. 
Urgencies implement the mechanism of self-composition in a new way, by executing choices out-of-program-order. 
The advantage is that the urgent choices are harmonized with the control flow, while the quantifiers in hyper model checking are resolved without synchronization. 
As we show, this harmony yields decidability results for analyzing urgency programs even with recursion, while hyper model checking has been shown to be undecidable despite a visibility assumption. 
In the appendix, we argue that the harmony enforced by urgency programs is justified from an application perspective. 


Compared to the above contributThis work is limited to finite words but supports
%
%
The work presented here is limited to finite words, but supports the new urgency annotations. 
%
On the conceptual level, it shows that the semantic domain can be derived from a study of the operators, Appendix~\ref{Appendix:Denotational}. 


Our axiomatization indeed induces a denotational semanti
Since the denotational semantics is expected to be compositional, this resembles the specialized contextual equivalence we study. 
In 
Indeed, our axiomatization directly induces a denotational 
The denotational semantics is expected
The landmark result is that 
One of the Salvati and Walukiewicz succeeded in giving a semantics capturing the full higher-order model-checking problem~\cite{SalvatiW15b}. 

 at hand (whether the program satisfies the 
assign  to the program a denotational semantics that answers the verification problem at hand (of whether the program satisfies the specification).



Our full abstraction results differ from these works not 

Characteristic terms, related to \cite{MP71}. 


These languages have been the basis for deciding contextual equivalence over first and second-order programs. 
The work of Murawski et al. have worked out a complete picture of the decdability status of contextual equivalence for higher-order languages. 
Combined with the full abstraction results, 
decidability and complexity 
In the cases of first-and second order programs, t
 results the for which we have proven full abstraction results 

Related work on contextual equivalence. 
Should be many results on full abstraction via game semantics. 

Related work on deciding contextual equivalence due to Murawski. 

Deciding making an observation. 
\begin{comment}
The field started with  Aehlig's work~\cite{Aehlig07} on denotational semantics for the safety verification of higher-order recursion schemes. 
%expressed in terms of (divergence-insensitive) non-deterministic tree automata with trivial acceptance (TAC automata in the following).  
%
He already formulated the difference with the Scott-Strachey approach: the semantics should capture \emph{"how this subterm 'looks, as seen by~$A$'"}, where $A$ is the specification. 
%
Terui~\cite{Terui12} studied the complexity of model-checking problems for the lambda calculus using denotational semantics with cleverly trimmed domains.  
%
The term \emph{effective denotational semantics} is due to Salvati and Walukiewicz~\cite{SalvatiW15}.
%
They showed that extremal fixed-point semantics capture precisely Boolean combinations of safety properties. 
%
%the properties expressible by Boolean combinations of divergence-insensitive TAC automata.
%
Moreover, they gave a denotational semantics for model checking against divergence-sensitive automata.
%
%It uses a product domain and a non-extremal fixed point. 
%The approach was generalized to weak monadic second-order logic in~\cite{SalvatiW17}.
%
With a different approach, Salvati and Walukiewicz succeeded in giving a semantics capturing the full higher-order model-checking problem~\cite{SalvatiW15b}. 
%
%Here, the domain is enriched by priorities and the semantics is a nested fixed point.
%
Recent work generalizes the correspondence to a model with visible priorities~\cite{Walu19}. 

An unexpected contribution to the field is due to Grellois and Melli\`es.
They noticed a tight link between the intersection type system for higher-order model checking~\cite{KobayashiOng2009} and linear logic~\cite{GM14}. 
%Indeed, a function application can be understood as duplicating an argument a number of times and consuming each copy once.
%Then turn Kobayashi Ong into a type system over linear logic.
Linear logic has different models, which can then be used to interprete types.
%This in turn leads to an interpretation of terms. 
%, namely as subsets of the interpretation of the corresponding types. 
In \cite{GM15b}, Grellois and Melli\`es study a qualitative model where the base type is interpreted as a set of states.
%This corresponds to idempotent intersection types.
The crux is to handle the parity condition.
The authors observe that a color is a modality and furnish an unconventional fixed-point operator %(on the colored qualitative lattice) 
inspired by the notion of runs in automata theory. 
The approach is powerful enough to solve the logical selection problem (cf. below).
In \cite{GM15}, Grellois and Melli\`es study a quantitative model of linear logic where the base type is interpreted as a multiset of states.
%This corresponds to non-idempotent intersection types. 
The domain gives information about the resources consumed by the verification process.
%It does not yield decidability.  
%The authors show that a collapse on the quantitative model results in the qualitative model.
Grellois's thesis identifies further links between higher-order model checking and linear logic~\cite{Grellois2016}.
%Resource-Management of the automaton. REL=SCOTTL without multiplicities.
%Denotations of Lambda with Resources.


Related %to effective denotational semantics 
is also Hofmann and Chen's type-theoretic approach to model checking recursive programs against linear-time specifications~\cite{Hofmann2014}. 
At the heart is the construction of a finite lattice out of the given B\"uchi automaton. %, an idea that goes back to~\cite{DHL06}. 
%The elements in this lattice abstract the program computations in a way that is sound and complete wrt. the specification. 
The authors give operators that mimic finite and infinite iteration on the abstract lattice. 
%With the domain at hand, they devise a type system that is sound and, assuming a suitable typing environment, also complete for the model-checking task. 
%Such an environment can again be computed as a fixed point.
In \cite{Hofmann2017}, the approach is generalized to functional programs.
The challenge is to interprete greatest fixed points of higher-order functions.
The key observation is that infinite iteration makes functions affine.

The works discussed above focus on verification. 
%
They consider infinite computations but are limited to demonic and perfect choice operators. 
%
Effective denotational semantics for angelic choice operators in finite computations have been developed in~\cite{HMM2016,HMM2017}.
%
Imperfect choices have not been considered, neither in denotational semantics nor from the perspective of equational reasoning.


Related work on axiomatization.

Related work on denotational semantics. 

Related work on imperfect information. 


Distributed synthesis considers an architecture and a specification with the goal to determine system components that together realize the specification~\cite{PR90}. 
The main result in this line of work is a characterization of the architectures for which the synthesis problem is decidable~\cite{FinkbeinerSchewe2005}. 
%Unfortunately, the positive results are limited to pipeline-like architectures. 
%Bounded synthesis offers a pragmatic way out, by synthesizing programs up to a size bound~\cite{FS13}. 
Finkbeiner and Olderog~\cite{FO17} studied games played over the unfoldings of Petri nets. 
The difference with distributed synthesis is the way information arises. %in the implementation of information. 
%way information is re
%This model implements information in a new way. 
%The motivation to shift the formulation is the way informedness is implemented.
In distributed synthesis, information is due to communication. 
In unfolding games, information is due to causality. 
In our setting, information is due to decisions.  
%The model is closer to an implementation
%Note that the related approaches rely on distribution as a means of implementing informedness. 
%We consider a sequential programming model instead, to which we add a mechanism of hiding choices. 
%The latter is easy to realize in structural operational semantics. %~\cite{SOS}. 
As we demonstrate, a sequential programming model gives better algorithmic results.
Imperfect information also arises in the distributed variant of Ramadge-Wonham controller synthesis~\cite{RamadgeWonham1987}. 
In this formulation, plant and controller should be implemented by asynchronous automata.
Decidability is still open (cf.~\cite{AWZ2009}), though there has been progress on unifying decidability results for fragments~\cite{HG17}. 
The challenge is to aggregate distributed information in a finite way. 
In our recursive language, there is no aggregation.
% -----------------------------------------------------------
% -----------------------------------------------------------
% -----------------------------------------------------------
% -----------------------------------------------------------
\subsubsection*{Graph Games}
Urgency games are related to pushdown games for which Walukiewicz showed a reduction to finite-state games~\cite{Walukiewicz2001}, based on procedure summaries~\cite{SharirPnueli1978}. 
Cachat showed that the winning region can be represented by an alternating automaton~\cite{Cachat2002}, using saturation~\cite{BEM97}.
The approach has been generalized to games over (collapsible) higher-order pushdowns in~\cite{BCHS12}. 
Kupfermann and Vardi reduced pushdown games to emptiness in alternating tree-walking automata~\cite{KV00}.
Also games over context-free grammars have been considered~\cite{MSS06,Bjorklund2013,Schuster16,Schuster17}.

None of the above models supports imperfect information. 
Pushdown games with imperfect information~\cite{Aminof2013} were studied in the context of model checking open systems~\cite{KVW01}. 
The problem is undecidable, despite a sequential programming model. 
Even perfect information about the stack height does not yield decidability~\cite{Bozelli2011}.
In our setting, the imperfect choices are part of the control flow. 
This compatibility is what yields decidability. 


\end{comment}




==> soundness_unused.tex <==
consider 
$\acontext{\contextvar}$ that is immediate for 
$\bot$ or $\aterm$.
%
Per definition, a context can only be immediate for a term
 if it
becomes an outermost subterm upon insertion.
%
Terminals are never rewritten, so an outermost terminal
remains outermost for the rest of the play.
%
Then Eve cannot win from $\acontext{\bot}$, because all strings of 
terminals $\atermp$ that can be reached from this position contain 
$\bot\not\in\analph$ which 
implies $\atermp\not\in\objective\subseteq\analph^{*}$.
%
The implication trivially holds.


==> todos.tex <==
\todo{Mention that urgency 1 is already the study of alternation/angelic and demonic choice. 
We are not aware of results on the contextual equivalence of this established programming model. 
Urgency 1 is also the formulation of (regular and context-free) perfect-information games with regular winning objectives. Not much is known about a compositional treatment of that model. }

\todo{Push through the example all the way. We have not shown the syntactic congruence on words, and we have not illustrated the decision procedure. }
\rfm{consider this done}

\todo{Hyper model checking encoding from simulation and language inclusion. Eve wins if inclusion fails. Product}

\todo{Ordinal theory in the appendix. }

\todo{Side condition on infinite replacement.}

\todo{Existence of ordinal for Eve winning.}

\todo{Make sure we have details from soundness in the appendix.}

\todo{Make sure we have right-separating proofs in the appendix.}

==> unused_extras.tex <==
%%%%% Some extras from axiomatization
The soundness of the identity axiom $\rmident$ and the associativity axiom $\rmassoc$ is intuitive.
%
The rewriting relation does not alter the terminals or the brackets in 
the top level concatenation.
%
The occurrences of the symbol $\ident$ and the order of the brackets have no effect on whether a word is in the objective.
%
These facts cause a similarity beyond $\congeq$-equivalence: The unrolled game trees are bisimilar.
%
For this reason, we will treat the terms like monoid elements, i.e. we will ignore or add brackets and $\ident$-symbols
where it is convenient.
%
The full proof can be found in the appendix.

Using the monoidal rules, we can see that if a term is immediate for a context $\acontext{\contextvar}$, 
the context is of the form $\acontext{\contextvar}=\atermppp\appl\contextvar\appl\atermpppp$.
%
Furthermore, it must hold that $\atermppp$, $\aterm$, and $\atermpppp$ are all terminal or 
$\urgencyof{\atermppp}<\urgencyof{\aterm}$ and $\urgencyof{\atermpppp}\leq\urgencyof{\atermp}$.
%
So, we can reformulate the \Cref{Lemma:ContextLemma} as follows: 
Let $\atermppp\appl\aterm\appl\atermpppp\implies\atermppp\appl\atermp\appl\atermpppp$ 
for all $\atermppp,\atermpppp\in\terms$ such that 
$\urgencyof{\atermppp}<max\set{\urgencyof{\aterm}, \urgencyof{\atermp}, 1}$ or 
$\atermpppp\leq\set{\urgencyof{\aterm}, \urgencyof{\atermp}}$. Then $\aterm\congleq\atermp$.

%%%%% Some extras from completeness

Base Case $\anurg=0$:
\noindent

\begin{lemma}\label{Lemma:ExtentionStability}
    For all specifications $(\analph, \objective)$,
    their extentions $(\analphp, \objectivep)$, $\anurg\in\nat$
    and $\aterm,\atermp\in\gnfn{\anurg}^{\analph, \objective}$,
    we have that $\aterm\axleq^{\analph, \objective}\atermp$
    iff $\aterm\axleq^{\analphp, \objectivep}\atermp$
    and $\aterm\discleq^{\analph, \objective}\atermp$ 
    iff $\aterm\discleq^{\analphp,\objectivep}\atermp$ 
\end{lemma}

This follows from the observation that
the axioms that depend on the
specification are uneffected by extentions.
%
That all proofs are 
also uneffected can be formally proven by a
standart transfinite induction on 
the depth of proof trees. 


\begin{lemma}\label{Lemma:RightSepExtentions}
    For all $(\analph, \objective)$, 
    there is an
    extention $(\analphp, \objectivep)$ where $\analph^{*}$ 
    is right seperable.
\end{lemma}

For the moment being, assume that this is correct.
%
We want to show that
$\aterm\axleq^{(\analph, \objective)}\atermp$
implies $\aterm\discleq^{(\analph, \objective)}\atermp$.
%
Assume that $\aterm\axleq^{(\analph, \objective)}\atermp$ holds.
%
Then, per \Cref{Lemma:ExtentionStability}, 
$\aterm\axleq^{(\analphp, \objectivep)}\atermp$ must 
also hold.
%
The axiomatization is sound under any specification, so
$\aterm\congleq^{(\analphp, \objectivep)}\atermp$.
%
Since $\aterm$ and $\atermp$ are terms built from $\analph^{*}$ 
and $\analph^{*}$ right-seperable under $(\analphp, \objectivep)$,
the condition for completeness is satisfied. 
%
This implies $\aterm\discleq^{(\analphp, \objectivep)}\atermp$ 
and thus again per \Cref{Lemma:ExtentionStability}, 
$\aterm\discleq^{(\analph, \objective)}\atermp$.
%
This concludes the proof.

\Cref{Lemma:RightSepExtentions} also implies data independent 
completeness.
%


%% TODO: Under works

Intuitively, one can extend the 
alphabet by special symbols of the form 
$[\aletter]\in\analphp$ for all $\aletter\in\analph$.
%
The word $\aword\in\analphp^{*}$ is in the objective iff
the symbols from $\analph$ form a word $\awordp$ and 
the symbols from $\analphp\setminus\analph$ form a word 
$\awordpp$ with $\awordpp\congleq^{\analph, \objective}\awordp$.


The proof sketch is as follows.
%
The leading term must be the leftmost term among outermost
actions with the highest urgency.
%
This can be thought to induce a strict total ordering on
outermost actions (also dependent on their positions in the context).
%
If the inserted term is paused, then it isn't ``maximal'' with 
respect to this ordering or it is enclosed by a choice.
%
This means that the maximal element, and thus the leading term,
remains unchanged, unless the inserted term is 
contained by the leading term.
%
In this case, the leading term is a choice.
%
Excluding the one successor that contains the inserted subterm,
the successors will be identical between the two terms.
%
Furthermore, that pair of successors 
will only differ at the inserted term.
%
So the successors can be expressed in terms of contexts 
enclosing the inserted terms.
%
This is exactly what the lemma states.







%
Let $\mathcal{L}_{\astate}
=\encoding{s_{0}, ..., s_{n-1}}^{\anurg-1}_{\astate}$ 
and $\mathcal{R}^{\astate} 
=\encoding{s_{n+1}, ..., s_{k}}^{\anurg}$.
%
A move is mirrored by the following steps.\\
%
\begin{tikzpicture}
    \tikzstyle{level 1}=[sibling distance=4.5em, level distance=15mm]
    \node[draw=none] 
    {$\mathcal{L}_{\astate}\appl 
    \makeleading{X} ... \$^{\anurg}\appl\mathcal{R}$}
    child {
        node[draw=none] {$\mathcal{L}_{\astate}\appl 
        \assertvar{s_{\anurg}}{\astate}\appl
        \makeleading{\encoding{\transitions_{\astate, X}}^{\anurg}}
        ... \$^{\anurg}\appl\mathcal{R}$}
        child {node[draw = none] 
        {$\mathcal{L}_{\astate}\appl 
        \assertvar{s_{\anurg}}{\astate}\appl
        \makeleading{\encoding{t}^{\anurg}}
        ... \$^{\anurg}\appl\mathcal{R}$} edge from parent[solid, ->]
            child{node[draw = none] {$\mathcal{L}_{\astate}'\appl 
            \assertvar{s_{\anurg}}{\astate}\appl
            \makeleading{Z}
            ... \$^{\anurg}\appl\mathcal{R}'$} edge from parent[dashed]}
        }
        edge from parent[dashed, ->]
    };
\end{tikzpicture}


























The encoding of a configuration is the concatentation 
of the encodings of the individual stacks, with a
few extra conditions.
%
For a stack $\sigma\$\in\Gamma^{+}$, we write
$\encoding{\sigma\$}^{\anurg}$
to denote an encoding term
$\stacksep\appl
\sigma_{0}^{\anurg}...\sigma_{n}^{\anurg}\appl\$^{\anurg}$,
ignoring the terminals except those in $\stacksep$.
%
We write $\encoding{s_0, ..., s_n}^{\anurg}$ to 
denote $\encoding{s_0}^{\anurg}...\encoding{s_n}^{\anurg}$.
%
We let
$\encoding{s_{0}, ..., (\astate, \anurg):s_{n},..., s_{k}}
=H^{\anurg-1}\appl
\encoding{s_{0}, ..., s_{n-1}}^{\anurg - 1}_{\astate}\appl
\encoding{s_{n}, ..., s_{k}}^{\anurg}\appl \stacksep$
where the terminals build a term that results in no 
assertion fails, no terminals of round $\leq \anurg - 1$ 
(except those in $@$), and consistent first states, i.e.
$f_{\anurgp}=s_{\anurgp + 1}$ for all $\maxurg>\anurgp\geq\anurg$.

First, remark that a symbol from a round only generates terminals 
that effect that round's variables.
%
For a term $H^{\anurg-1}\appl
\encoding{s_{0}, ..., s_{n-1}}^{\anurg - 1}_{\astate}\appl
\encoding{s_{n}, ..., s_{k}}^{\anurg}\appl \stacksep$,
we have $\urgencyof{H^{\anurg-1}\appl
\encoding{s_{0}, ..., s_{n-1}}^{\anurg - 1}_{\astate}}=\anurg-1$
and $\urgencyof{\encoding{s_{n}}^{\anurg}}=\anurg$.
%
This means that 
$H^{\anurg-1}\appl
\encoding{s_{0}, ..., s_{n-1}}^{\anurg - 1}_{\astate}\appl
\makeleading{\encoding{s_{n}}}^{\anurg}\appl
\encoding{s_{n+1}, ..., s_{k}}^{\anurg}
\appl\stacksep$.
%
The stack encoding is just a seperator followed by
the contents of the 
stack laid out in order, i.e.
$\encoding{s_{n}}^{\anurg}=\stacksep\appl\makeleading{\wrpsymbol{\anurg}}...\wrplsymbol{\anurg}$.
%
The leading term property follows from $\urgencyof{\stacksep}=0$.
%
A stack symbol, after being unwrapped, 
contains two choices, each guarded by an assertion.
%
Since we'd have $c_{\anurg}=\sty$ at this point of the run,
Eve must choose the second option, popping the stack symbol.
%
Then, the term that encodes the stack becomes 
$\stacksep\appl
\makeleading{\bigEchoiceOf{\anurg}_{\astate\in\states}
\assertvar{s_{\anurg}}{\astate}\appl
\encoding{\transitions_{\astate, \stsymbol}}^{\anurg}}...\wrplsymbol{\anurg}$
%
Here, each of Eve's choices are guarded by an assertion about the 
current state.
%
This forces Eve to choose $\astate\in\states$ that 
corresponds to the current state.
%
In this case, the game becomes 
$\stacksep\appl
\assertvar{s_{\anurg}}{\astate}\appl
\encoding{\transitions_{\astate, \stsymbol}}^{\anurg}...\wrplsymbol{\anurg}$
%
This is equal to
$\stacksep\appl
\assertvar{s_{\anurg}}{\astate}\appl
\makeleading{
\bigPchoiceOf{\anurg}_{\atrans\in\transitions_{\astate, \stsymbol}}
\encoding{\atrans}^{\anurg}}
...\wrplsymbol{\anurg}$,
where the owner of the state chooses an applicable transition.
%
In the case of the usual pop/push operations, 
the result is the encoding of the configuration 
that would be reached by this transition.
%
For example, if the transition popped $\stsymbol$ and pushed 
$\stsymbolp\appl\stsymbolpp$ while going from $\astate$ to 
$\astatep$, we'd have 
$\stacksep\appl
\assertvar{s_{\anurg}}{\astate}\appl
\setvar{s_{\anurg}}{\astatep}\appl
\wrpsymbolp{\anurg}\appl\wrpsymbolpp{\anurg}
...\wrplsymbol{\anurg}$.
%
The case of a stack generation is equivalent to 
pushing an extra stack seperator, which also results in 
the relevant encoding term:
$\stacksep\appl
\assertvar{s_{\anurg}}{\astate}\appl
\setvar{s_{\anurg}}{\astatep}\appl
\wrplsymbol{\anurg}\appl\stacksep\appl
...\wrplsymbol{\anurg}$
%
The term $\stacksep\appl
\assertvar{s_{\anurg}}{\astate}\appl
\setvar{s_{\anurg}}{\astatep}\appl
\wrplsymbol{\anurg}$ encodes the new stack.
%
The context switching transition sets the 
control variable $c_{\anurg}$ to $\nxt$, i.e.
$\stacksep\appl
\assertvar{s_{\anurg}}{\astate}\appl
\setvar{s_{\anurg}}{\astatep}\appl\setvar{c_{\anurg}}{\nxt}\appl
\makeleading{\wrpsymboln{0}{\anurg}}...
\wrpsymboln{a}{\anurg}\appl\wrplsymbol{\anurg}$,
where $s_n=\stsymboln{0}\appl...\appl\stsymboln{a}$.
%
The next stack symbol becomes leading, which lets Eve 
make a choice.
%
Since at this point $c_{\anurg}=\nxt$, the 
guards force her to choose the first option.
%
This writes a lower urgency version of the same stack symbol 
in the old one's place: 
$\stacksep\appl
\assertvar{s_{\anurg}}{\astate}\appl
\setvar{s_{\anurg}}{\astatep}\appl\setvar{c_{\anurg}}{\nxt}\appl
\assertvar{c_{\anurg}}{\nxt}
\wrpsymboln{0}{\anurg-1}\appl\makeleading{\wrpsymboln{1}{\anurg}}...
\wrpsymboln{a}{\anurg}\appl\wrplsymbol{\anurg}$.
%
The same thing happens here onwards, until the 
$c_{\anurg}$ is set back to $\sty$ at the next stack seperator.
%
Then the leading term shifts to the next stack.
%
So this term encodes the configuration reached after 
the context switch.
%
The only edge case is $n=k$, where there aren't any more 
stacks to the right that become leading.
%
In this case, the leading term becomes $H^{\anurg - 1}$
,which is at the start of the term.
%
This term allows Eve to set the first state of the 
round $\anurg - 1$, by generating the term
$H^{\anurg-2}
\appl\setvar{s_{\anurg-1}}{\astatepp}\appl\setvar{f_{\anurg-1}}{\astatepp}$.
%
Since this is the only position where Eve will get to set 
$f_{\anurg-1}$, and no new assignments for $s_{\anurg}$ 
will be generated, Eve must choose $f_{\anurg - 1}$ to be 
equal to the last $s_{\anurg}$ assignment, which 
is the resulting state of the transition $\astatep$.
%
So the state of the previous round becomes the 
state of the current round.
%
Since $\urgencyof{H^{\anurg - 2}}=\anurg - 2$, the top of 
the following stack becomes leading, initiating a new round.



%%%%%%%%%%%%%%%%%%%%
%Belongs in appendix
%%%%%%%%%%%%%%%%%%%%

Before moving on to the normalization, we state the 
lemma below. 
%
It will prove useful during the normalization process.
%
The correctness follows from the repeated application of (L6).

\begin{lemma}
    Let $\acontextdn{\anurg}{\contextvar}=
    \bigEchoiceOf{\maxurg}\set{\bigAchoiceOf{\maxurg}\set{...
    \bigEchoiceOf{\anurg+1}\set{\Achoice_{\anurg + 1}\set{\contextvar}}}}$ 
    for all $\anurg<\maxurg$ 
    and $\acontextdn{\maxurg}{\contextvar}=\contextvar$.
    %
    Then, for all $\aterm\in\gnfn{\anurg}$, we have 
    $\acontextdn{\anurg}{\aterm}\axeq\aterm$ and 
    $\acontextdn{\anurg}{\aterm}\in\gnfn{\maxurg}$.
\end{lemma}

Assume that this holds for all $\anurg,\anurgp\leq\maxurg$ 
with $\anurgp\leq\anurg$.
%
We can find the $\anurgp>\anurg$ case by simply letting 
$\normof{\bigPchoiceOf{\anurgp}\atermsetpp}=
\normof{\bigPchoiceOf{\anurgp}\set{\normof{\atermpp'}
\mid \atermpp'\in\atermsetpp}}$.
%
Since $\normof{\atermpp'}\in\gnfn{\maxurg}$ for all
$\atermpp'\in\atermsetpp$, the term size is multiplied 
by a factor of at most $\sgexpof{2\maxurg - 1}$.
%
So in total, the process takes 
$(\sgexpof{2\maxurg - 1})^{2}=\sgexpof{2\maxurg-1}$ time.

\todo{You are here}

\noindent\emph{Inductive step} $\anurg>\anurgp$:


\noindent This step is where the axioms $\rnormalform$ and its dual 
(NA) see use.
%
Remark that a trivial application of $\rlatassoc$ 
concludes 
$\bigPchoiceOf{\anurgpp}\atermset\axeq
\bigPchoiceOf{\anurgpp}\set{\bigPchoiceOf{\anurgpp}\atermset}$
for any $\anurgpp\leq\maxurg$.
%
We can combine this observation 
with the rules, along with (N) and (N1) to get the helper rule 
(N2):
\begin{align*}
    \axdef{(N2)}{}{
        \multiline{
            \bigEchoiceOf{\anurgp}_{k\in K}\bigPchoiceOf{\anurg}\atermsetppp_{k}
            \axeq\bigEchoiceOf{\anurgp}_{k\in K}\bigPchoiceOf{\anurgp}\atermsetppp_{k}
        }{
            \bigAchoiceOf{\anurgp}_{k\in K}\bigPchoiceOf{\anurg}\atermsetppp_{k}
            \axeq\bigAchoiceOf{\anurgp}_{k\in K}\bigPchoiceOf{\anurgp}\atermsetppp_{k}
        }
    }
\end{align*}
%
We use this rule while normalizing $\bigPchoiceOf{\anurgp}\atermsetpp$:
\begin{align*}
    \bigPchoiceOf{\anurgp}\atermsetpp
    \;=\;
    \bigPchoiceOf{\anurgp}_{i\in I}
        {\bigEchoiceOf{\anurg}{j\in J_{i}}
            {\bigAchoiceOf{\anurg}{}{\atermsetp_{i, j}} }}
    \axeqper{2\times\text{(N2)}}
    \bigPchoiceOf{\anurgp}_{i\in I}
        {\bigEchoiceOf{\anurgp}{j\in J_{i}}
            {\bigAchoiceOf{\anurgp}{}{\atermsetp_{i, j}} }}
    \label{Eq:ChoiceUrgencyClamping}\tag{n1}
\end{align*}
%
\noindent Remark that $\atermsetp_{i, j}\subseteq\gnfn{\anurg-1}$,
so we can apply the induction hypothesis to find 
$\atermppp_{i, j}\in\gnfn{\anurgp}$ with
$\atermppp_{i, j}\axeq\bigAchoiceOf{\anurgp}\atermsetp_{i, j}$.
%
We can then use the monotonity $\rlatassoc$ to replace the 
terms with their equivalents in the term.
%
We apply this argument exhaustively
with $\atermppp_{i}=\normof{\bigEchoiceOf{\anurgp}_{j\in J_{i}}\atermppp_{i, j}}$ 
and $\atermppp=\normof{\bigPchoiceOf{\anurgp}_{i\in I}\atermppp_{i}}$:
%
\begin{align*}
    \bigPchoiceOf{\anurgp}_{i\in I}
        {\bigEchoiceOf{\anurgp}{j\in J_{i}}
            {\bigAchoiceOf{\anurgp}{}{\atermsetp_{i, j}} }}
    \axeqper{\text{I.H.}}
    \bigPchoiceOf{\anurgp}_{i\in I}
        {\bigEchoiceOf{\anurgp}{j\in J_{i}}
            {\atermppp_{i, j}}}
    \axeqper{\text{I.H.}}
    \bigPchoiceOf{\anurgp}_{i\in I}
        {\atermppp_{i}}
    &\axeqper{\text{I.H.}}
    \atermppp\in\gnfn{\anurgp}
    \label{Eq:ChoiceInductionHyp}\tag{n2}
\end{align*}


%%%%%%%%%% Better Preliminaries


\subsection{Contextual Equivalence}
The notion of observable behavior is not compositional: we may have $\winsof{\aterm}{\objective}$ if and only if $\winsof{\atermp}{\objective}$ for all objectives~$\objective$, 
yet the two terms behave differently when placed into a context.
%
This is a common problem in semantics, and the way out is to consider the largest congruence that lives within observational equivalence.  
%
In our setting, this leads to the following definition which is key to our development. 
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
\begin{definition}
The \emph{contextual equivalence} $\approx\ \subseteq \terms\times\terms$ between urgency terms is defined by $\aterm\approx\atermp$, if 
\begin{align*}
\forall \acontext{\contextvar}\in \contexts.\ \forall \objective\subseteq\analph^*.\  \winsof{\aterm}{\objective} \text{ if and only if }\winsof{\atermp}{\objective}\ . 
\end{align*}
Let $\objective\in\analph^*$ be an objective. 
%
The \emph{$\objective$-specialized contextual equivalence} $\approx_{\objective}\ \subseteq \terms\times\terms$ is defined by $\aterm\approx_{\objective}\atermp$, if
\begin{align*}
\forall \acontext{\contextvar}\in \contexts.\  \winsof{\aterm}{\objective} \text{ if and only if }\winsof{\atermp}{\objective}\ . 
\end{align*}
\end{definition}
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------
% --------------------------------------------------------------------------------

We just defined two notions of contextual equivalence, the former universally quantifying over all objectives and the latter fixing an objective.
Both are common in the literature and well-justified. 
With an appropriate objective, the specialized contextual equivalence can be used to study the termination behavior of programs and termination with an error, as alluded to above. 
Contextual equivalence is more precise and takes into account the all observable behavior, in particular the outcome of a computation and the side-effects.
Both notions also have motivation from a verification perspective. 

Urgency terms can be used to model algorithmic problems as different as hyperproperty verification, language inclusion, and synthesis problems where program and environment have local information that is invisible to the other. 
%
The objective then serves as the specification to be met in a verification or synthesis task. 
%
Contextual equivalence gives information about which information can be abstracted away from an urgency term without influence on the objective, similar to how bisimilarity preserves the satisfaction of $\text{CTL}^*$ properties.

Having an infinite set of non-terminals and infinitary terms allows us to model parameterized functions in a simple yet general way. 
We not only introduce a non-terminal for each function, but a non-terminal for each instantiation of the function's formal parameters by actual values. 
Similarly, we can react on values using explicit and potentially infinite branching. 
This style of modeling stems from process algebra.
%
\Cref{Appendix:?} elaborates on the modeling aspect. 


To establish the full abstraction results, it will be convient to work with preorder variants of contextual equivalence that are defined as expected. 
The \emph{contextual preorder} $\aterm\preceq\atermp$ says that $\winsof{\aterm}{\objective}$ implies $\winsof{\aterm}{\objective}$ for all $\objective\subseteq\analph^*$. 
The \emph{$\objective$-specialized contextual preorder} $\aterm\preceq_{\objective}\atermp$ is $\winsof{\aterm}{\objective}$ implies $\winsof{\atermp}{\objective}$. 
The relationship with the above definitions is this.
% ------------------------------------------------------------------------
% ------------------------------------------------------------------------
% ------------------------------------------------------------------------
% ------------------------------------------------------------------------
\begin{lemma}\label{Lemma:Preorder}
(1) $\aterm\approx\atermp$ iff $\aterm\preceq\atermp$ and $\aterm\succeq\atermp$. 
(2) $\aterm\approx_{\objective}\atermp$ iff $\aterm\preceq_{\objective}\atermp$ and $\aterm\succeq_{\objective}\atermp$.
\end{lemma}
% ------------------------------------------------------------------------
% ------------------------------------------------------------------------
% ------------------------------------------------------------------------
% ------------------------------------------------------------------------


==> upper_bound_unused.tex <==
\begin{comment}
In this section, we provide a sketch of an
algorithm for solving a regular urgency game.
%
The algorithm is an effective denotational semantics 
algorithm that is based on the methods developed in
\Cref{Section:Normalization}.
%
It relies on a normal form of finite size,
which is not the case in \Cref{Section:Normalization}.
%
So we modify the normal form in the direction of the 
specialized precongruence.
%
Observe that the equivalence classes of $\axeq$ on 
$(\analph\cup\set{\bot})^{*}$ make up $\gnfn{0}$, which is
the normal form for urgency $0$.
%
We extend this approach to the specialized precongruence.
%
Only $\rabsbot$ and $\rtequiv$ apply to terminal strings.
%
We can see that $\rtequiv$ is broader than $\rabsbot$ for any 
$\objective\subseteq\analph^{*}$.
%
So for the objective $\objective\subseteq\analph^{*}$, 
we define $\specgnfn{0}$ as 
the equivalence 
classes of the relation 
$\lreq{\objective}=\;\lrleq{\objective}\cap\lrgeq{\objective}$
on $(\analph\cup\set{\bot})^{*}$.
%
Since $\objective$ is regular, $\specgnfn{0}$ is finite.
%
The construction for the higher urgency normal forms 
$\specgnfn{\anurg>0}$ and $\specagnfn{\anurg>0}$  
remain the same relative to the normal forms they reference.
%
So we have $\specgnfn{\anurg>0}=
\set{\bigEchoiceOf{\anurg}\atermset\mid 
\emptyset\neq\atermset\subseteq\specgnfn{\anurg - 1}}$
and $\specagnfn{\anurg>0}=
\set{\bigAchoiceOf{\anurg}\atermset\mid
\emptyset\neq\atermset\subseteq\specagnfn{\anurg}}$.
%
Note that since
$\specgnfn{0}$ is finite,
$\specgnfn{\maxurg}$ and all the intermediary 
sets are also finite.
\end{comment}


At the lowest level
needs a twist 
that is unique to the specialized contextual preorder and does not apply to the contextual preorder. 
The twist is to refine the normal form. 


calls for a twist. 

 according to the $\objective$-specialized axiomatic precongruence, $\normof{\aterm}\specaxleq{\objective}\normof{\atermp}$. 
However, the very same method would also be able to decide the contextual preorder, which we have just seen is undecidable, \Cref{Proposition:Undec}. 
T

the undecidability results in \Cref{Proposition:Undec,Theorem:UndecSpec}. 
It requires a twist, though, with the following reasoning. 

In the ligh
The normal forms as defined above cannot always (and typically will not) be finite, for otherwise we would have a contradiction to 
The problem is that the normal form terms on the lowest level are all words over $\analphbot$, which form an infinite set. 
To remedy

There is a twist, how

We provide an algorithm to compare two terms according to a fixed special the upper bound in Theo



The algorithm follows the idea outlined above: compute the normal forms of the given terms and compare them according to the specialized axiomatic precongruence. 
The undecidability result in \Cref{Proposition:Undec}, however, shows that the idea cannot work out of the box. 
What fails is that normal form terms as defined in \Cref{Section:Normalization} are typically infinite, 
and therefore neither computable nor comparable. 
The source of this infinity can be found in the base case: already $\gnfn{0}=\analph^*\cup\set{\bot}$ is infinite, and this propagates upwards. 
The way out is to realize that the $\objective$-specialized axiomatic congruence allows us to further factorize this set using \Cref{axiom:spec}. 
The resulting so-called $\objective$-specialized normal form is guaranteed to yield finite terms (and finitely many of them).   
We turn to the details. 


The first step is to break this 
The goal is to decide 
The full abstraction result in \Cref{Theorem:FullAbstractionSpecialized}: $\aterm\speccongleq{\objective}\atermp$ iff $\aterm\specaxleq{\objective}\atermp$. 
With \Cref{Proposition:EffDenSemUpperBound}, we can replace the terms by their normal forms: 
$\aterm\specaxleq{\objective}\atermp$ iff $\specnormof{\aterm}\specaxleq{\objective}\specnormof{\atermp}$. 
On normal form terms, the axiomatic precongruence coincides with the domination preorder, \Cref{Lemma:DominationPreorder} and \Cref{Proposition:Soundness}. 
We thus have: $\specnormof{\aterm}\specaxleq{\objective}\specnormof{\atermp}$ iff $\specnormof{\aterm}\discleq\specnormof{\atermp}$. 
The domination preorder is easy to check, namely in non-deterministic polyni has hte  which is easier to handle algorithmi

Here, the

The decision procedure 


%In the 
%only quadratically many classes in the syntactc whose objective has only quadratically many classes.
%
%In the following, we elaborate

%The modification propagates to all terms and use  $\specgnfnof{\maxurg}{\arrobjective}$ to refer to the corresponding terms in normal form. 
%
%Herr, $\arrobjective$ is a new objective obtained from $\objective$ by replacing each transition $\transitions(\astate,\aletter) = \astatep$ by $\transitions(\astate, (\astate, \astatep)) = \astatep$, and adding transitions to create a DFA.
%
The key observation is that 
%
O
This propagates upwards and we obtain 
The key insight 


$\atermpp\appl\contextvar\appl\atermppp$ are easy to represent: they are the upward closure wrt. $\specaxleq{}$  of so-called \emph{characteristic terms}.  the number of soluatire are not so many solution spaces. 


The idea 
This is made po

 is the insight that 
Interestingly, the solution spaces of contexts $\atermpp\appl\contextvar\appl\atermppp$ are easy to represent: they are the upward closure wrt. $\specaxleq{}$  of so-called \emph{characteristic terms}.  the number of soluatire are not so many solution spaces. 

Now, this key insight is that the solution space of a context is easy to represent algorithmically. 

%is the upward closure of a 

%
Hence, when two contexts have the same solution space, the same set of terms $\aterm$ for which $\winsof{\acontext{\aterm}}{\objective}$.


%
%
Interestingly, this equivalence among contexts can be captured through the novel concept of \emph{characteristic terms}. 
%


 $\atermpp$ and check $\atermpp \specaxleq{\objective} \aterm$ resp. $\atermpp \specaxleq{\objective} \atermp$. 


 if for every term 
The job of a context is to tell terms a
If for eIf two co
Intuitively, two context
 is  
We have 
The number of contexts to be considered is quadratic in the size of~$\specgnfn{\maxurg}$.
Whether Eve has a winning strategy on a normal form term can be checked in polynomial time by saturating from the leaves to the root.



\begin{comment}

The complexity of the normalization process depends on 
the size of $\specgnfn{0}$.
%
The following definition helps us make this precise.
%
\begin{definition}\label{Definition:TowerFunctions}
    Let $\objective\subseteq\analph^{*}$ be regular.
    %
    We define $\sgexpof{0}=\bigoof{|\specgnfn{0}|}$ 
    and $\sgexpof{\anurg + 1}=2^{(\sgexpof{\anurg})}$.
\end{definition}
The \Cref{Proposition:EffDenSemUpperBound}
states the upper bound for the complexity of the normalization.
%
Remark that 
$\max\set{|\aterm|\mid \aterm\in\gnfn{\maxurg}}=\sgexpof{2\maxurg-1}$.
%
This is because the set $\gnfn{\maxurg}$ is constructed by applying 
the power set construction $\maxurg$ times.
%
For any $\aterm\in\specgnfn{\maxurg}$, 
the winner can be decided in $\bigoof{|\aterm|}=
\bigoof{\sgexpof{2\maxurg-1}}=\sgexpof{2\maxurg-1}$ time.
%
So, after normalization, solving the game is trivial.
%
The overall complexity dominates $\sgexpof{2\maxurg-1}$,
so the complexity of 
solving a game from $\aterm$ using this approach is also
$|\aterm|\cdot\sgexpof{2\maxurg-1}+
|\eqmap|\cdot|\nonterminals|\cdot\sgexpof{2\maxurg-1}$.

Note that in the worst case we have 
$|\specgnfn{0}|\sim 2^{|\adfa|}$.
%
So directly applying the algorithm from 
\Cref{Proposition:EffDenSemUpperBound}
gets us a $\kexptime{2\maxurg}$ algorithm.
%
To reduce the complexity, we employ a polynomial time reduction 
beforehand.
%
The reduction ensures that $|\specgnfn{0}|$ is polynomial in $|\adfa|$.
%
\Cref{Lemma:PolynomialSemigroup} makes this formal.

\begin{lemma}\label{Lemma:PolynomialSemigroup}
    Let $(\nonterminals, \eqmap, \adfa, \aterm)$ 
    be a regular urgency game with the $\dfa$ 
    $\adfa=(\astate_{0}, \states, \analph, \transitions, 
    \goalstates)$.
    %
    We can construct a winning-equivalent 
    instance 
    $(\nonterminals', \eqmap', \adfa', \aterm')$ over $\analph'=\transitions$
    in polynomial time
    where $(\analph'\cup\set{\bot})^{*}$ has at 
    most $|\states|^{2}+1$ many
    $\lreq{\langof{\adfa'}}$-classes 
\end{lemma}

The construction involves replacing each $\aletter\in\analph$
by $\bigEchoiceOf{1}\set{(\astate, \aletter, \astatep)\in\transitions}$ 
in $\aterm$ and $\eqmapof{\nonterminal}$ for all 
$\nonterminal\in\nonterminals$. 
%
Intuitively, instead of reaching 
$\aword\in(\analph\cup\set{\bot})^{*}$ 
Eve constructs the run $\aword$ has
in $\mathcal{A}$.
%
The language of accepting runs has at most 
$|\states|^{2}+1$ equivalence classes.
%
Eve loses
if the string of transitions do not form a run in 
$\mathcal{A}$, so she is forced to construct a valid run.
%
The full proof can be found in the appendix.
\end{comment}

%admit another algorithm that is interesting for several reasons. 
%It brings together the semantic results obtained so far, and exploits them algorithmically.
%It is more efficient, though the benefit is not large enough as to change the worst-case upper %bound. 
%The algorithm is based on the idea sketched in the beginning. 



% ------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------
\subsection{Right-Separating Objectives}
For right-separating objectives, we can give a simpler algorithm that does not iterate over contexts.  
We use the full abstraction result in \Cref{Theorem:FullAbstractionSpecialized} to translate the problem  $\aterm\speccongleq{\objective}\atermp$ into $\aterm\specaxleq{\objective}\atermp$. 
Then we apply \Cref{Proposition:EffDenSemUpperBound} to replace the terms by their $\objective$-specialized normal forms.
The $\objective$-specialized normal form terms are also in the normal form of \Cref{Section:Normalization}. 
Hence, the axiomatic precongruence coincides with the domination preorder, \Cref{Lemma:DominationPreorder} and \Cref{Proposition:Soundness}. 
The latter has the advantage of being easier to handle algorithmically.
The following proposition summarizes the reasoning.
% -----------------------------------------------------------------------------------
% -----------------------------------------------------------------------------------
% -----------------------------------------------------------------------------------
% -----------------------------------------------------------------------------------
\begin{proposition}\label{Proposition:DecProcRightSeparating}
Let $\objective$ be right-separating and $\aterm, \atermp$ finitary. 
Then we have $\aterm\speccongleq{\objective}\atermp$ if and only if $\specnormof{\aterm}\discleq\specnormof{\atermp}$. 
\end{proposition}
% -----------------------------------------------------------------------------------
% -----------------------------------------------------------------------------------
% -----------------------------------------------------------------------------------
% -----------------------------------------------------------------------------------
Our algorithm is thus to compute $\specnormof{\aterm}$ and $\specnormof{\atermp}$, which takes time $\maxurg$-fold exponential only in the objective. 
Then we decide the domination preorder on the resulting normal form terms, which can be done in polynomial time. 

==> verification_unused.tex <==

Instead, it should be possible to evaluate Now, if we also assume the terms to be finite,   
ThThe full abstraction results are motivating wh gets rid of the universal quantifier over contexts in the definition of the contextual preorder resp. the $\objective$-specialized variant. 
Therefore, it is natural to ask whether the relations become decidable, if study the decidability and complexity status of these rels ask whether these relations bec may be there may be hope for
 con
\begin{theorem}
For finitary terms, 
\end{theorem}



Using the domain shattering objectives introduced earlier, there will be non-regular sets $\objective$ for which the specialized contextual equivalence $\speccongeq{\objective}$ is undecidable.
We show a stronger result: no matter which objective $\objective$ is chosen, if it is non-regular, then $\speccongeq{\objective}$ will be undecidable.
\begin{theorem}\label{Theorem:UndecSpec}
\decwhichover{\speccongeq{\objective}}{\maxurg} is undecidable for every $\maxurg$ and every non-regular $\objective$. 
\end{theorem}
The universal quantifier over the objective is unhandy in an undecidability proof. 
Our approach to deal with it is as follows, inspired by~\cite{todo}. 
If $\objective$ is non-regular, then it has infinitely many classes. 
These classes can be brought into a linear order and thus embed the natural numbers. 
We use this observation to encode Minsky machines.

\begin{comment}
\begin{definition}\label{Definition:ObjectLengths}
    The size $|\aterm|$ of a term $\aterm\in\terms$
    is the size of its formula tree, i.e 
    $|\aterm\appl\atermp|=|\aterm|+|\atermp|+1$ and 
    $|\bigPchoiceOf{\anurg}\atermset|=1+\sum_{\aterm\in\atermset}|\aterm|$.
    %
    The size of an assignment 
    $\eqmap:\nonterminals\to\terms$
    is the collective size of the image of $\eqmap$, 
    so we have $|\eqmap|=
    \sum_{\nonterminal\in\nonterminals}|\eqmapof{\nonterminal}|$.
\end{definition}
\end{comment}



In this section, we study the complexity of 
solving a concrete urgency game.
%
We restrict our focus to regular urgency games.
%
A regular $\maxurg$-urgency game
is an urgency game with a finitary starting term, 
finitary defining term assignments,
maximal choice urgency $\maxurg$, and a
regular objective.
%
We make these notions precise in
\Cref{Section:UBPreliminaries}.
%
\Cref{Theorem:Complexity} states our main result.

\begin{theorem}\label{Theorem:Complexity}
    Deciding the winner of a 
    regular $\maxurg$-urgency game is 
    $\kexptime{(2\maxurg - 1)}$ complete.
\end{theorem}

The upper bound is by effective
denotational semantics.
%
The algorithm is based on the methods
developed in \Cref{Section:Normalization}.
%
We make them effective and efficient. 
%
The lower bound is by reduction from Multi Pushdown Games, 
a model for the synthesis of concurrent programs.
%
Using urgency carefully, 
it is possible 
to control which part of the term becomes
leading.
%
We use this to model 
two independent stacks under boundedly many context
switches.


\subsection{Upper Bound Preliminaries}\label{Section:UBPreliminaries}
We define a concept of length for terms and defining 
term assignments.
%
\begin{definition}\label{Definition:ObjectLengths}
    The size $|\aterm|$ of a term $\aterm\in\terms$
    is the size of its formula tree, i.e 
    $|\aterm\appl\atermp|=|\aterm|+|\atermp|+1$ and 
    $|\bigPchoiceOf{\anurg}\atermset|=1+\sum_{\aterm\in\atermset}|\aterm|$.
    %
    The size of an assignment 
    $\eqmap:\nonterminals\to\terms$
    is the collective size of the image of $\eqmap$, 
    so we have $|\eqmap|=
    \sum_{\nonterminal\in\nonterminals}|\eqmapof{\nonterminal}|$.
\end{definition}

A finitary term is a term $\aterm$ with $|\aterm|\in\nat$.
%
Similarly, a finitary assignment $\eqmap:\nonterminals\to\terms$
is an assignment with $|\eqmap|\in\nat$.
%
Note that if the assignment $\eqmap:\nonterminals\to\terms$
is finitary, we also have $|\nonterminals|\in\nat$.

We can now formally define regular 
urgency games.
%
A \emph{regular $\maxurg$-urgency game} 
over $\analph$ is a tuple
$(\nonterminals, \eqmap, \adfa, \aterm)$ 
that consists of
a finite set of non-terminals 
$\nonterminals$, a function $\eqmap:\nonterminals\to\terms$
that assigns each non-terminal a finitary term, a 
DFA $\adfa=(\states, \astate_{0}, 
\analph, \transitions, \goalstates)$ 
that accepts the winning objective, and 
a finitary starting term $\aterm\in\terms$.
%
In $\aterm$ and $\eqmapof{\nonterminal}$ 
for all $\nonterminal\in\nonterminals$,
the maximal choice urgency is $\maxurg$.
%
The regular $\maxurg$-urgency game instance 
$(\nonterminals, \eqmap, \adfa, \aterm)$ defines a
game from $\aterm$ with objective $\langof{\adfa}$ and 
defining term assignments $\eqmap:\nonterminals\to\terms$.


We argue that there is hope for positive findings as follows. 
The full abstraction results we have just proven remove the universal quantification over contexts in the definition of these relations.
Moreover, they give us a normal form for the axiomatic congruence that is free from recursion. 
Therefore, it should be possible to decide $\aterm\congleq \atermp$ resp. $\aterm\speccongleq{\objective}\atermp$ by computing the normal form terms $\normof{\aterm}$ and~$\normof{\atermp}$ and comparing them using the (specialized) axiomatic precongruence. 


